Manifold Graph Signal Restoration using Gradient Graph Laplacian Regularizer

In the graph signal processing (GSP) literature, graph Laplacian regularizer (GLR) was used for signal restoration to promote piecewise smooth / constant reconstruction with respect to an underlying graph. However, for signals slowly varying across graph kernels, GLR suffers from an undesirable "staircase" effect. In this paper, focusing on manifold graphs -- collections of uniform discrete samples on low-dimensional continuous manifolds -- we generalize GLR to gradient graph Laplacian regularizer (GGLR) that promotes planar / piecewise planar (PWP) signal reconstruction. Specifically, for a graph endowed with sampling coordinates (e.g., 2D images, 3D point clouds), we first define a gradient operator, using which we construct a gradient graph for nodes' gradients in sampling manifold space. This maps to a gradient-induced nodal graph (GNG) and a positive semi-definite (PSD) Laplacian matrix with planar signals as the 0 frequencies. For manifold graphs without explicit sampling coordinates, we propose a graph embedding method to obtain node coordinates via fast eigenvector computation. We derive the means-square-error minimizing weight parameter for GGLR efficiently, trading off bias and variance of the signal estimate. Experimental results show that GGLR outperformed previous graph signal priors like GLR and graph total variation (GTV) in a range of graph signal restoration tasks.

==> 2nd-response2reviewers/defs.tex <==
\def\0{{\mathbf 0}}
\def\1{{\mathbf 1}}

\def\a{{\mathbf a}}
\def\b{{\mathbf b}}
\def\c{{\mathbf c}}
\def\d{{\mathbf d}}
\def\e{{\mathbf e}}
\def\f{{\mathbf f}}
\def\g{{\mathbf g}}
\def\h{{\mathbf h}}
\def\i{{\mathbf i}}
\def\j{{\mathbf j}}
\def\k{{\mathbf k}}
\def\l{{\mathbf l}}
\def\m{{\mathbf m}}
\def\n{{\mathbf n}}
\def\o{{\mathbf o}}
\def\p{{\mathbf p}}
\def\q{{\mathbf q}}
\def\r{{\mathbf r}}
\def\s{{\mathbf s}}
\def\t{{\mathbf t}}
\def\u{{\mathbf u}}
\def\v{{\mathbf v}}
\def\w{{\mathbf w}}
\def\x{{\mathbf x}}
\def\y{{\mathbf y}}
\def\z{{\mathbf z}}

\def\A{{\mathbf A}}
\def\B{{\mathbf B}}
\def\C{{\mathbf C}}
\def\D{{\mathbf D}}
\def\E{{\mathbf E}}
\def\F{{\mathbf F}}
\def\G{{\mathbf G}}
\def\F{{\mathbf F}}
\def\H{{\mathbf H}}
\def\I{{\mathbf I}}
\def\J{{\mathbf J}}
\def\K{{\mathbf K}}
\def\L{{\mathbf L}}
\def\M{{\mathbf M}}
\def\N{{\mathbf N}}
\def\O{{\mathbf O}}
\def\P{{\mathbf P}}
\def\Q{{\mathbf Q}}
\def\R{{\mathbf R}}
\def\S{{\mathbf S}}
\def\T{{\mathbf T}}
\def\U{{\mathbf U}}
\def\V{{\mathbf V}}
\def\W{{\mathbf W}}
\def\X{{\mathbf X}}
\def\Y{{\mathbf Y}}
\def\Z{{\mathbf Z}}


\def\rE{{\text{E}}}
\def\rPr{{\text{Pr}}}
\def\Tr{{\text{Tr}}}
\def\vec{{\textrm{vec}}}
\def\ie{{\textit{i.e.}}}
\def\eg{{\textit{e.g.}}}


\def\cA{{\mathcal A}}
\def\cB{{\mathcal B}}
\def\cC{{\mathcal C}}
\def\cD{{\mathcal D}}
\def\cE{{\mathcal E}}
\def\cF{{\mathcal F}}
\def\cG{{\mathcal G}}
\def\cH{{\mathcal H}}
\def\cI{{\mathcal I}}
\def\cK{{\mathcal K}}
\def\cL{{\mathcal L}}
\def\cM{{\mathcal M}}
\def\cN{{\mathcal N}}
\def\cO{{\mathcal O}}
\def\cP{{\mathcal P}}
\def\cQ{{\mathcal Q}}
\def\cR{{\mathcal R}}
\def\cS{{\mathcal S}}
\def\cT{{\mathcal T}}
\def\cU{{\mathcal U}}
\def\cV{{\mathcal V}}
\def\cW{{\mathcal W}}
\def\cX{{\mathcal X}}
\def\cY{{\mathcal Y}}
\def\cZ{{\mathcal Z}}


\def\bpi{{\pmb{\pi}}}
\def\bphi{{\pmb{\phi}}}
\def\bpsi{{\pmb{\psi}}}
\def\bphi{{\pmb{\phi}}}
\def\bpsi{{\pmb{\psi}}}
\def\balpha{{\boldsymbol \alpha}}
\def\bbeta{{\boldsymbol \beta}}
\def\bmu{{\boldsymbol \mu}}
\def\btheta{{\boldsymbol \theta}}
\def\bupsilon{{\pmb{\upsilon}}}
\def\bvarphi{{\boldsymbol \varphi}}
\def\bGamma{{\boldsymbol \Gamma}}
\def\bLambda{{\boldsymbol \Lambda}}
\def\bPhi{{\boldsymbol \Phi}}
\def\bOmega{{\boldsymbol \Omega}}
\def\bPsi{{\boldsymbol \Psi}}
\def\bSigma{{\boldsymbol \Sigma}}
\def\bTheta{{\boldsymbol \Theta}}


\def\bcdot{{\;\boldsymbol{\cdot}\;}}

==> 2nd-response2reviewers/reviewer_2.tex <==
{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 1:}

With all due respect, it seems that the authors are confused by the mathematical terminology. Namely, different results used in ANY paper can be called Facts/ Claims/ Propositions/ Lemmas(Lemmata) and, finally, Theorems. These terms all refer to TRUE and (maybe) IMPORTANT results but they play different roles. Namely, any result that is called a Theorem without name of person like Stokes' Theorem or citation is by default claimed to be proven by the authors and to be the main or one on the main contributions of the article. If the authors claim that Theorem 1 is the main result and it has never been known before then the paper must be rejected. This result is definitely known. The authors might look it up in any basic Linear Algebra course. However, if the authors just want to mention it and use as an auxiliary result, they have to call it a Fact/Property/Lemma. For example, Schur's Lemma is an extremely important and even central result in representation theory but everybody calls it lemma. From here we see that being a lemma doesn't mean the result is unimportant.

If the authors insists that Theorem 1 is their theorem (they never cite a source) then the paper must be rejected.  
}\vspace{\comafter}



\noindent\textbf{Response 1:}
With due respect to the reviewer, we are not sure this discussion is productive in the context of a paper review; we should be discussing the \textit{content} of lemmas and theorems rather than the \textit{definitions} of lemmas and theorems. 
Nonetheless, for the sake of completeness, we have looked up the Merriam-Webster dictionary, and ``lemma" is defined as 
\vspace{0.1in}
\begin{quote}
An auxiliary proposition used in the demonstration of another proposition\footnote{https://www.merriam-webster.com/dictionary/lemma}.  
\end{quote}
In contrast, a ``theorem" is defined as
\begin{quote}
A formula, proposition, or statement in mathematics or logic deduced or to be deduced from other formulas or propositions\footnote{https://www.merriam-webster.com/dictionary/theorem}.
\end{quote}
These definitions are consistent with our understanding and usage in our manuscript, namely, lemma 1 and 2 are foundational pieces we first introduced from which Theorem 1 is built later.

The reviewer appears to focus exclusively on the first part of Theorem 1 stating that the GNG Laplacian is positive semi-definite (PSD) (note that a reference to a standard linear algebra book by Golub and Van Loan \cite{Golub2013MatrixC} is added). 
However, the second part of the Theorem stating that planar signals are the $0$ frequencies of the GNG Laplacian---and thus the GGLR signal prior is promoting (biasing the solution towards) planar signal reconstruction---is entirely neglected. 
If the reviewer insists this part is also known in the literature, we humbly ask the reviewer to provide a reference. 

Finally, we note again that through multiple rounds of reviews, we have received technical comments only about Theorem 1 by this reviewer, while the vast majority of the paper has received no comments.
We humbly ask the reviewer again to read the \textit{entire} manuscript and provide a balanced critique of the whole work.

\vspace{\resafter}



{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 2:}
For the Ridge Regression issue, i am pasting here a link to Wikipedia page https://en.wikipedia.org/wiki/Ridge$\_$regression. The title of this link speaks for itself. This page among other facts and concepts is talking about EXACTLY your situation. They call it Tikhonov regression and it might be viewed as a type or close relative of Ridge Regression. 

In any case, if the authors insist that they wont cite the source and want still to call it a Theorem, the paper must be rejected.
}\vspace{\comafter}

\noindent\textbf{Response 2:}
We first humbly remind the reviewer that, in the first review round, the reviewer wrote that our equation (31) of Theorem 3 is the same as ``ridge regression".
As we have already explained in our response 3 to reviewer 2 in the first round, \textit{Theorem 3 (equation (1) below) is not the same as ridge regression (equation (2) below)}:
\begin{align}
\x^* &= \left( \H^\top \H + \mu \cL \right)^{-1} \H^\top \y 
\label{eq:thm3} \\
\hat{\beta}_R &= \left( \X^\top \X + \lambda \I \right)^{-1} \X^\top \y
\label{eq:rr} .
\end{align}
As anyone can plainly see, the two equations are \textit{not} the same when GNG Laplacian matrix $\cL$ in \eqref{eq:thm3} (which is positive semi-definite (PSD)) is not the same as the identity matrix $\I$ in \eqref{eq:rr} (which is positive definite (PD)). 
\textbf{The important implication is that coefficient matrix $\X^\top \X + \lambda \I$ in \eqref{eq:rr} is guaranteed to be PD and invertible, while $\H^\top \H + \mu \cL$ is not.}
This necessitates the need for Theorem 3 and proof in Appendix C, from which we have received no comments from the reviewer in two review rounds.

In this review round, the reviewer now doubled down and stated that our Theorem 3 is the same as ``Tikhonov regression". 
First, there is no such thing as ``Tikhonov regression"; we conjecture that the reviewer means ``Tikhonov regularization" instead. 
Second, it is known that the reviewer's cited Wiki-page is incorrect\footnote{See a discussion of this Wiki-page error here. https://stats.meta.stackexchange.com/questions/4305/is-tikhonov-regularization-really-a-synonym-for-ridge-regression} in stating that ``ridge regression" is the same as ``Tikhonov regularization". 
Instead, Tikhonov regularization is
\begin{align}
\hat{\x} = (\A^\top \A + \bGamma^\top \bGamma)^{-1} \A^\top \b.
\end{align}
Thus, \textbf{Tikhonov regularization is a \textit{super-set} that includes ridge regression as a special case when matrix $\bGamma = \I$} (see equation (2.1) in \cite{Hoerl2000RidgeRB} for ridge regression and equation (3) in \cite{Golub1999TikhonovRA} for Tikhonov regression). 
Decomposing PSD GNG Laplacian $\cL$ into $\cL = \bGamma^\top \bGamma$, 
%where $\bGamma = \sqrt{\bSigma} \U^\top \R \G$ (using the much abused Theorem 1), 
indeed the equation (3) in Theorem (1) can be viewed as a special case of Tikhonov regularization. 
But so is previously proposed \textit{graph Laplacian reglarizer} (GLR) \cite{pang17}, $\x^\top \L \x$, and \textit{graph shift variation} (GSV) \cite{romano17}, $\|(\I - \A) \x\|^2_2$, and \textit{left eigenvectors of the random walk graph Laplacian} (LeRaG) \cite{liu17}, $\x^\top \L_{rw}^\top \L_{rw} \w$ (where $\L_{rw}$ is the random walk Laplacian), and so on. 
Each of these specialized Tikhonov regularizations has its own spectral properties, and thus promotes (bias the solutions towards) different signal reconstruction. 
So, what exactly is the problem here? 
In our case, we proved in Theorem 1 that GGLR promotes (bias the solution towards) planar signal reconstruction (\ie, planar signals are the $0$ frequencies of GNG Laplacian $\cL$).
We also provided detailed analysis in Theorem 3 specifying under precisely what conditions when matrix $\H^\top \H + \mu \cL$ is full-rank and invertible.
To the best of our knowledge, these theorems do not exist previously in the literature. 
Instead of an unreliable wiki-page, we humbly ask the reviewer for a precise reference if we are incorrect.

\vspace{\resafter}



==> 2nd-response2reviewers/reviewer_3.tex <==
{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 1:}
I thank the authors for the revised manuscripts where they have attempted to answer many of my comments and questions. The manuscript is much more easy to follow, and specially some of the definitions are more explicit than before.
}\vspace{\comafter}

\noindent\textbf{Response 1:}
We thank the reviewer for the positive comment.

\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 2:}
The authors now provide a definition of a K-dimensional planar signal on page 4. However, we are not still told what the relation between the the different $\alpha$’s of the plane can be, specially in connection to it being a graph signal.

More importantly, we are led to next the definition of a [piecewise planar signal, which forms the crux of the work. However, it still remains unclear what a general piece-wise planar signal means. Yes, the authors have provided an example of a 1D linear signal. But how this extends to even the next dimension is unclear. Basically, what defined a notion of piecewise planar - what is meant by ‘adjacent sub-domains’? The authors state ‘If one further assumes signal
…then the two adjunct linear pieces must coincide’. How is adjacency defined, even qualitatively? And what does it mean to coincide? Please consider clarifying these concepts.
}\vspace{\comafter}


\noindent\textbf{Response 2a:}
Putting aside \textit{piecewise planar} notion and focusing on the simpler \textit{planar} notion, it appears that the reviewer is already confused between a \textit{continuous hyperplane} and \textit{discrete samples} on a hyperplane that compose a graph signal. 
Specifically, in the previous manuscript, we provided a definition of a continuous $K$-dimensional \textit{hyperplane} (equation (6) in the revised manuscript), which is common in the literature. 
$\alpha$'s are the standard parameters that define the hyperplane---like slope $m$ and $y$-intercept $b$ for a one-dimensional linear line $y=m x + b$---parameter vector $\balpha$ is the \textit{manifold gradient}. 
%A discrete signal on a manifold graph is a collection of discrete samples on a continuous manifold, each with coordinate in the manifold space. 
A collection of discrete samples residing on the same hyperplane is a planar discrete signal; connecting neighboring samples via edges results in a planar graph signal. 
This is very clearly illustrated in Fig.\;3(a) in the revised manuscript, where there are four discrete samples on the same 2D plane. 
This seems rather straightforward, and we failed to understand the reviewer's confusion.

\vspace{0.2in}
\noindent\textbf{Response 2b:}
The notion of neighboring sub-domains or sub-graphs is common in the graph literature---see, for example, \textit{nodal domain theorem} \cite{Bykoglu2005NodalDT}. 
For the sake of completeness, we provide a definition here and in the revised manuscript. 
In our context, we define a \textit{sub-domain} $\cN_m$ as a maximally connected subset of nodes $i$ such that the corresponding discrete samples $x_i$ reside on the same hyperplane.
We assume that nodal domains are non-overlapping.
Two nodal domains $\cN_m$ and $\cN_n$ are \textit{adjacent} if there exist at least one node $i \in \cN_n$ and one node $j \in \cN_m$ such that $\exists (i,j) \in \cE$. 
We failed to understand the reviewer's confusion, since piecewise constant (PWC) graph signal---where samples in each sub-domain evaluate to the same constant---is well discussed in the GSP literature \cite{pang17,liu17}, and PWP graph signal---where samples in each sub-domain reside on the same hyperplane---is just a natural extension. 

\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 3:}
In Response to my comment 3, the authors attempt to demonstrate the fallacy of the argument’ - I am not sure what the fallacy is referred to here. Also, the authors demonstrate that $(\x-\A \x)^{\top}\L(\x-\A \x)$ is not small by considering a particular example of a pathological graph which is a line graph whose starting and end nodes have only one connection, the rest all have two neighbours. The entire arguments falls short if this is instead considered for a path graph or a ring graph. So it is not right to say that my argument is entirely fallacious.

Further, the authors choose a particular signal x=[2, 0, -1], instead if you consider a graph of larger number of nodes, but the same linear signal, say running from -2 to 2 in steps of 100 (100 nodes), the measured quantity again will be zero only at the two extreme nodes, and in this is similar to the edge-effects well known in discrete  signal processing. I do not think this refutes the validity of my suggestion of using $(\x-\A \x)^{\top}\L(\x-\A \x)$ as a meaningful way to enforce smoothness of the derivative or the residual leading to piecewise planar regularisation.

Further in the response 3, the authors mention ‘which agrees with our intuition for a linear line’ What is a linear line?

Also they state ‘The reason we can compute a more reasonable regularizer for a linear line is because we computed manifold gradients w.r.t. latent coordinates that are defined globally’ -  this was not clear - is it reasonable because you used latent coordinates that had nothing to do with the actual graph?

Again, after all the newer additions, the motivation for the PWP and indeed the formulation itself seems ill-posed.
}\vspace{\comafter}

\noindent\textbf{Response 3a:}
First, we are puzzled that the reviewer continued to insist on $(\x - \A \x)^\top \L (\x - \A \x)$ as a reasonable regularizer to promote some notion of graph linearity when a counter-example was already provided in our previous response. 
A theorem is proven false when a single counter-example is given; counter-intuitively, the reviewer seems content with a proposal that may work only part of the time (and remains unclear when it would work and to what extent in general). 
In particular, what constitute ``extreme nodes" in a general graph is very unclear: given a finite graph with nodes of varying node degrees, what are the ``extreme nodes" according to the reviewer? 
For a general graph then, how does the reviewer propose to account for ``edge-effects" without first correctly identifying the so-called ``extreme nodes"? 
This is hardly sound algorithm design as an engineering principle. 
In contrast, our GGLR proposal to promote planar / PWP graph signals, based on fast computation of graph embedding to obtain latent coordinates for each node, does not require identification of ``extreme nodes" and works every time. 

Moreover, in the previous revised manuscript we have already demonstrated definitively why using $(\L \x)^\top \L (\L \x)$ to promote signal linearity, where $\L \x$ is used to compute \textit{graph gradients}, is not reasonable. 
The reviewer's suggestion of $\x^\top (\I - \A)^\top \L (\I - \A) \x = (\L_n \x)^\top \L (\L_n \x)$, where normalized graph Laplacian $\L_n = \D^{-1/2} \L \D^{-1/2}$ is used to compute graph gradient $\L_n \x$ instead of $\L \x$, is just a normalized variant of the same idea. 
We have already indicated in a footnote (footnote 9 in the revised manuscript) that a similar argument can be made for other versions of graph Laplacians.
Nonetheless, for the sake of completeness, we now show in detail why this normalized variant is also not reasonable.
(This is included in Appendix A in the revised manuscript.)

We begin by showing that the only signal that computes to $(\L_n \x)^\top \L (\L_n \x) = 0$ is $\x = \v_1 = \text{diag}(\D^{1/2})$, where $\v_1$ is the (unnormalized) first eigenvector corresponding to eigenvalue $0$ for $\L_n$. 
First, it is obvious that $(\L_n \v_1)^\top \L (\L_n \v_1) = 0$, since by definition of eigenvector $\v_1$ corresponding to eigenvalue $\lambda_1 = 0$, $\L_n \v_1 = \D^{-1/2} \L \D^{-1/2} \text{diag}(\D^{1/2}) = \D^{-1/2} \L \1 = \0$.
Second, in order for $\y^\top \L \y = 0$ where $\y \neq \0$, $\y$ must be the constant signal $c\1$ that is the (unnormalized) first eigenvector corresponding to eigenvalue $0$ of $\L$.
In general, any vector $\x = \sum_{n=1}^N \alpha_n \v_n$ can be expressed as a linear combination of eigenvectors $\{\v_n\}$ of $\L_n$ that are orthogonal basis vectors spanning the signal space $\cH = \mathbb{R}^{N}$, where $\alpha_i = \langle \x, \v_i \rangle = \v_i^\top \x$. 
We now write
\begin{align}
\L_n \x &\stackrel{(a)}{=} \left( \sum_{i=2}^N \lambda_i \v_i \v_i^\top \right) \left(\sum_{n=1}^N \alpha_n \v_n \right) \\
&\stackrel{(b)}{=} \sum_{i=2}^N \lambda_i \alpha_i \v_i
\end{align}
where in $(a)$ we write symmetric matrix $\L_n$ as a linear combination of rank-1 matrices that are outer-products $\v_i \v_i^\top$ of its eigenvectors $\v_i$, each scaled by eigenvalue $\lambda_i$. 
$(b)$ follows since eigenvectors of symmetric matrix $\L_n$ are orthogonal, \ie, $\v_i^\top \v_j = \delta_{i-j}$. 
Note importantly that there is no $\v_1 \v_1^\top$ in the summation, since $\lambda_1 = 0$. 

Thus, in order for $\y^\top \L \y = 0$, $\y$ must equal $c\1 = \L_n \x = \sum_{i=2}^N \lambda_i \alpha_i \v_i$.
However, we see that inner-product $\langle c\1, \v_1 \rangle = \v_1^\top c \1 = c \sum_i v_{1,i} = c \sum_i d_i^{1/2}$, where $d_i > 0$ is the degree of node $i$ for a positive connected graph $\cG$. 
Thus, $\sum_i d_i^{1/2} > 0$, and $c \sum_i d_i^{1/2} \neq 0$ for $c \neq 0$. 
Given $\langle c \1, \v_1 \rangle \neq 0$, constant signal $c\1$ cannot be written as $c \1 = \sum_{i=2}^N \lambda_i \alpha_i \v_i$, except for the case when $c=0$ and $\alpha_i = 0, \forall i$. 
We can therefore conclude that the only signal $\x$ such that $(\L_n \x)^\top \L (\L_n \x) = 0$ is $\x = \v_1$, the first eigenvector of $\L_n$.  
However, this means that the dominant signal (lowest frequency) $(\L_n \x)^\top \L (\L_n \x)$ is promoting is exactly the same as $\x^\top \L_n \x$.
Hence, the reviewer's suggested $(\L_n \x)^\top \L (\L_n \x)$ promotes signal construction that is essentially no different from existing GLR $\x^\top \L_n \x$ using a normalized graph Laplcian $\L_n$. 


Further, it is clear that even the constant signal $\x = c \1$, which has zero gradient and is thus smooth and linear in any reasonable definition of signal linearity, does not compute to zero, \ie, $0 \neq (\L_n c \1)^\top \L (\L_n c \1)$.
We can thus concclude that $(\L_n \x)^\top \L (\L_n \x)$ is not a reasonable regularizer to promote graph signal linearity.

\begin{figure}
\centering
\begin{tabular}{c}
\includegraphics[width=6.2in]{long version/fig/reviewer_comparison.png}
\vspace{-0.1in}
\end{tabular}
\caption{Image patch denoising using three different priors: SDGLR, SDGGLR, and the reviewer's suggested prior $(\L_n \x)^\top \L (\L_n \x)$. We observe that the suggested prior is noticeably worse than the proposed SDGGLR.}
\label{fig:reviewer_suggestion}
%\vspace{-0.1in}
\end{figure}

We have conducted an experiment on image denoising to demonstrate that the reviewer's suggested regularizer $(\L_n \x)^\top \L (\L_n \x)$ did indeed perform noticeably worse than our proposed SDGGLR, as shown in Fig.\;\ref{fig:reviewer_suggestion} here, agreeing with our understanding. 
We see that in the second image, the reviewer's suggestion performed even worse than previous SDGLR with noticeable false contours due to its inability to promote even a simple constant signal. 

\vspace{0.1in}
\noindent
\textbf{Response 3b:}
Since the reviewer explicitly asked ``what is a linear line", a concept studied in elementary school, we provide a definition below for the sake of completeness.
A one-dimensional function $f(x)$ is a linear line with respect to independent variable $x$ if $f(x)$ can be written as $f(x) = a x + b$, where $a, b \in \mathbb{R}$ are the slope and $y$-intercept of the line, respectively.
We refer the reviewer to this Wiki page\footnote{https://en.wikipedia.org/wiki/Linear\_equation} for details.
We are puzzled by this comment as well, since the reviewer appears to understand this concept when discussing ``a graph of larger number of nodes but the same linear signal" earlier. 

\vspace{0.1in}
\noindent 
\textbf{Response 3c}:
We vehemently disagree with the reviewer's claim that the latent coordinates ``had nothing to do with the actual graph". 
The latent coordinates of a graph are computed via our proposed fast \textit{graph embedding} method with linear time $\cO(N)$ complexity described in Section VI. \textit{Graph embedding}---a well studied topic in the machine learning literature \cite{LLE, LE} for over a decade---computes coordinates in a low-dimensional space, where Euclidean distances between computed coordinates correspond to node-to-node network distances in the original graph. 
Saying our computed latent coordinates ``had nothing to do with the actual graph" shows a lack of basic understanding of what a graph embedding actually is. 
We humbly ask the reviewer to peruse overview papers in graph embedding such as \cite{hamilton17, xu21} for reference.

\vspace{0.1in}
\noindent
\textbf{Response 3d:}
In summary, in this response 3, the reviewer has i) insisted on a ill-advised regularizer $(\L_n \x)^\top \L (\L_n \x)$ that promotes the same dominant signal construction as conventional GLR $\x^\top \L_n \x$ and hence does not promote any new notion of ``graph linearity" (and experimentally performed noticeably worse than our proposed GGLR); ii) questioned what a linear line is---a concept taught in elementary school; and iii) demonstrated a lack of basic understanding of what a graph embedding is.
In totality,  with due respect to the reviewer, this does not amount to a technically sound argument why our formulation, described in Section\;IV for signals with coordinates and Section\;VI for signals without coordinates, is ``ill-posed". 
We humbly ask the reviewer to reread Section\;IV and VI carefully for a basic understanding of our formulation.

\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 4:}
In response 4, they mention ‘As discussed in the Introduction and shown in new Fig.1, many graph signals are slowly varying across the underlying kernels, and promoting PWC signal reconstruction is clearly not suitable. This motivates a generalization to promote PWP signal reconstruction instead ’  — what are these kernels? Alternatively, given the example in Figure (b) could you visualise the benefits of your approach over regular GLR? Given that the work is for general graph signals and it is a mostly empirical work, it is not sufficient to just lift the motivation from image setting and make it a motivation for graphs. 
}\vspace{\comafter}

\noindent\textbf{Response 4:}
In the revised manuscript, we have reconstructed Fig.\;1 to show the denoising results of temperature signals on a China geographical graph (kNN graph for $k=5$). 
It consists of 3191 nodes, and each node represents a regional district in China. 
The data comes from Loess Plateau SubCenter, National Earth System Science Data Center, National Science \& Technology Infrastructure of China\footnote{http://loess.geodata.cn}.
Kindly note that this is not an image setting, and the graph is not a regular kernel such as a 2D grid. 
In Fig.\;1 of the revised manuscript (Fig.\;\ref{fig:PWP_ex1} here), we can clearly observe the ``staircase" effect---artificial signal discontinuities between adjacent reconstructed constant sub-domains---for SDGLR.
In contrast, our proposed SDGGLR produced a much smoother signal reconstruction and higher PSNR.

\begin{figure}
\centering
\begin{tabular}{c}
\includegraphics[width=6in]{long version/fig/tmp2.png}
\vspace{-0.1in}
\end{tabular}
\caption{Examples of staircase effects. We can see denoising results (PSNR) using SDGLR and SDGGLR on the corrupted temperature graph with noise variance 50. The staircase effect of SDGLR, as compared to SDGGLR, is visually obvious.}
\label{fig:PWP_ex1}
%\vspace{-0.1in}
\end{figure}
\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 5:}
Response 5: ‘There exist many practical graph signals that are slowly varying across the underlying kernels with occasional discontinuities;
 Again, as I mention above, then why don’t the authors give us concrete examples of such graph signals instead of referring to TV and TGC that are used in a 2D setting which has also visual or perceptual motivation, whereas this is not the case in graphs? Why is stair-case effect relevant for graphs? Does it affect the compression of graph signals, for example?

Also, a question that I had in mind from the discussion on K-planar signals: Does the eigenvectors basis, K-of them in particular, form a suitable basis for the K-planar signal space? In that case, can you connect your work to a K-band-limited graph signal setting?

Further, given a general setting of a graph and graph signals, how do I judge if the latent coordinates obtained by your approach in Section VI is ‘good’? This is particularly for settings where the graph is not a 2D image… 
}\vspace{\comafter}

\noindent\textbf{Response 5a:}
For motivation, in Fig.\;1 of the revised manuscript (Fig.\;\ref{fig:PWP_ex1} here) we have already included an example of a non-imaging signal that is slowly varying across the underlying graph kernel---temperature signal on a China geographical graph.
Staircase effect is an undesirable artifact that introduces artificial signal discontinuities across adjacent reconstructed constant sub-domains, while the ground-truth signal is smooth---the problem is not unique to images.
This is clearly demonstrated in Fig.\;\ref{fig:PWP_ex1}(c) for temperature signal in China, in Fig.\;\ref{fig:PWP_ex2}(d) for a synthetic smooth signal on a manifold graph, and Fig.\;\ref{fig:PWP_ex3}(c) for a 3D point cloud, when conventional SDGLR was used. 
These artifacts would appear for the graph version of TV called \textit{graph total variation} (GTV) as well \cite{elmoataz08,couprie13}.
These observable staircase artifacts are not only visually unpleasant; they lead to erroneous signal reconstructions, resulting in lower PSNR (larger MSE) compared to our proposed SDGGLR. 
We are unsure what is the relevance of staircase effects to signal compression, which is outside the scope of this paper focusing on signal restoration.


\vspace{0.2in}
\noindent\textbf{Response 5b:}
The whole point of the proposed GGLR $\x^\top \cL \x$ using new matrix GNG Laplacian $\cL$ is that \textit{any} planar graph signal $\x$ with discrete samples residing on the same hyperplane will evaluate to $\x^\top \cL \x = 0$; in other words, \textbf{planar signals are the $0$ frequencies of PSD GNG Laplacian matrix $\cL$}. 
In term of eigen-analysis, \textit{all planar signals reside in a $K$-dimensional eigen-subspace corresponding to the smallest eigenvalue $\lambda_1 = 0$ of $\cL$ with multiplicity $K$.} 
This is analogous to the constant signals that are the $0$ frequencies of the PSD graph Laplacian matrix $\L$; here, the 1-dimensional eigen-subspace spanned by the constant vector $\1$ corresponds to the smallest eigenvalue $\lambda_1 = 0$ of $\L$ with multiplicity $1$. 
In the revised manuscript, we have made this point explicit in the Introduction and in Theorem\;1 to facilitate understanding.

Note that by formulating a MAP optimization problem of the following form (equation (30) in the revised manuscript) for signal reconstruction:
\begin{align}
\min_\x \|\y - \H \x\|^2_2 + \mu \,\x^\top \cL \x
\end{align}
we are only biasing the signal reconstruction towards low frequencies of $\cL$, instead of a strict bandlimited signal reconstruction as done in bandlimited sampling, for example \cite{anis16}.
See \cite{cheung18} for details of general MAP formulations and associated spectral interpretations for graph signal reconstruction. 


\vspace{0.2in}
\noindent\textbf{Response 5c:}
The reviewer is essentially asking about quality evaluation of any computed graph embedding.
In the graph embedding literature \cite{hamilton17, xu21}, the quality of a computed graph embedding (coordinates for each graph node) is evaluated for specific graph applications. 
We have conducted extensive experiments to test our embedding method in our earlier conference version of this work \cite{Chen2022DSLW}, focusing exclusively on graph clustering. 
We compared it with representative state-of-art embedding methods: LLE\;\cite{LLE}, LE\;\cite{LE}, DeepWalk\;\cite{DeepWalk}, node2vec\;\cite{node2vec}, and NetWalk\;\cite{NetWalk}. 
To evaluate clustering accuracy, we used four criteria: Rand Index (RI), Precision, Purity, and Normalized Mutual Information (NMI) \cite{Alok2013DevelopmentOA}. 
Experiments show that our embedding is among the fastest in the literature, while producing the best clustering performance for manifold graphs. 
Due to page limitation, here we only compared our embedding method for GGLR in the experimental section with two representative embedding methods, LLE and LE. 
We observe that our embedding method achieves the best interpolation performance for manifold graphs.

\vspace{\resafter}

\begin{figure}
\centering
\begin{tabular}{c}
\includegraphics[width=6in]{long version/fig/rollgraph.png}
\vspace{-0.1in}
\end{tabular}
\caption{We conducted an experiment on a synthetic manifold graph. We first uniformly sampled 3000 points from a continuous manifold surface, and then constructed a kNN manifold graph ($k=5$). The original noiseless graph is shown in (a). The zoom-out version and its corrupted version are in (b) and (c), respectively. We can observe staircase effects in (d) due to SDGLR. The result by our proposed SDGGLR looks smoother in (e).}
\label{fig:PWP_ex2}
%\vspace{-0.1in}
\end{figure}
\vspace{\resafter}

\begin{figure}
\centering
\begin{tabular}{c}
\includegraphics[width=5in]{long version/fig/man.png}
\vspace{-0.1in}
\end{tabular}
\caption{Denoising results using SDGLR and SDGGLR on the corrupted 3D point cloud \textit{MAN} with noise variance 25. As we can see the staircase effect in (c) is caused by SDGLR. The result by SDGGLR looks more natural in (d).}
\label{fig:PWP_ex3}
%\vspace{-0.1in}
\end{figure}
\vspace{\resafter}

{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 6:}
Response 7: the authors state that in ‘For graphs that do not naturally have latent coordinates as attributes, and they are not manifold graphs, then reasonable latent coordinates cannot be easily obtained using our proposed method’ it would be nice to clarify what reasonable is meant, and how the user can judge it for a new dataset - for example if all I have access to is graph and signals on graph, how do I judge if the manifold representation you present is ‘reasonable’ or effective? In the end, we are talking about a basis representation of graph signals, and then the eigenspace of the laplacian or GGLR  or SDGLR forms the basis for expressing the signals (PWP, for example). 
}\vspace{\comafter}

\noindent\textbf{Response 6a:}
For the question of ``when is a graph a manifold graph?", we have already provided a criterion in the paper in Section VI, which we repeat here for completeness. 
Given a graph composed of nodes uniformly sampled from a smooth manifold, the betweenness centrality of nodes should be similar, \ie, all nodes are equally likely to appear in a given shortest path.
Thus, we first divide each $C_B(i)$ by the number of $(s,t)$ pairs, $(N-1)(N-2)$, and then employ the \textit{variance of betweenness centrality} (VBC) as a metric to evaluate the quality of a manifold graph. 
Only qualified manifold graphs are inputted to our algorithm to compute embeddings. 
As shown in Table II, the first four graphs with smaller VBCs are considered as qualified manifold graphs. 

%Note that the notion that a combinatorial graph is a collection of random samples on \textit{one} low-dimensional manifold is one assumption on strcture within the data, and like all structure model assumptions on data (\eg, sparse coding, low-rank matrices), they are not always (approximately) true. 

\vspace{0.1in}
\noindent\textbf{Response 6b:}
As previously discussed, the eigen-subspace corresponding to the smallest eigenvalue $\lambda_1 = 0$ of multiplicity $K$ is the set of planar graph signals. 
This is precisely why $\x^\top \cL \x = 0$ for all planar signals $\x$, 



\vspace{\resafter}

{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 7:}
Detailed response 9: isn’t that also true for the regular graph Laplacian? 
}\vspace{\comafter}

\noindent\textbf{Response 7:}
First, it should be clear that this is not true for the reviewer's proposed prior $(\L_n \x)^\top \L (\L_n \x)$, since $(\L_n \1)^\top \L (\L_n \1) \neq 0$, and thus the reviewer's proposed prior is \textit{not} invariant to constant shifts. 

Second, it is indeed true also for the regular combinatorial graph Laplacian $\L = \D - \W$, which is obvious since the first (unnormalized) eigenvector $\v_1$ corresponding to eigenvalue $0$ is the constant all-one vector $\v_1 = \1$, \ie, $\L \1 = \0$. 
Thus, it is very clear that a constant-shifted vector $\1 + c \1 = (1+c) \1$ is still constant, and thus $\L (1+c) \1 = (1+c) \L \1 = \0$. 

For the case of 1-dimensional GNG Laplacian $\cL$, the dimension of the eigen-subspace for eigenvalue $0$ is two, \ie, $\v_1 \perp \v_2$ and $\cL \v_1 = \cL \v_2 = \0$.
In this case, it is less obvious whether a constant shift of any vector $\u = a_1 \v_1 + a2 \v_2$ in this eigen-subspace automatically means $\cL (\u + c \1) = \0$.
We provided a proof here.

\vspace{\resafter}



{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 8:}
Detailed response 14 and in Remark under Theorem 2:
What is 1D GNG is not clearly defined (It appears first on page 8), is this the same as 1-dimensional PWP, with K=1? This was a bit unclear. Then is it the case that the signal at every node is of the form ($\x_i = a + b \p_i$) ? Is this what is meant by a linear signal referred to in the response and Remark2? Please clarify.
}\vspace{\comafter}

\noindent\textbf{Response 8:}
Due to the limited space available (only 16 pages are permitted for a revised TSP manuscript, including references), we have removed the discussion on 1D GNG Laplacian in the revised manuscript. 

\vspace{\resafter}



{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 9:}
Detailed response 18: Agreed, but the true value of optimal tradeoff is itself a function of the true $\x^o$ as can be seen from equation (33) - this seems a bit circular to me in that case.

Also, doesn’t modelling $\lambda_i$ as an exponential function implicitly mean that it is a low-pass graph signal? Then isn’t the following analysis restricted to that particular case of graph signals? On the other hand, the house signal does indeed have edges, and hence is not a smooth GS - I am a bit confused here. I request the authors to clarify this part.
}\vspace{\comafter}

\noindent\textbf{Response 9a:}
First, computing the optimal tradeoff between the fidelity term and a regularizer term in general is a well-studied topic in machine learning and signal processing---called the \textit{bias-variance tradeoff} \cite{Belkin2018ReconcilingMM}. 
Specifically for graph signal denoising and using GLR for regularization, it was investigated previously in \cite{chen2017bias}.
We are simply extending this analysis to the case when the regularizer is GGLR instead of GLR.
Specifically, we only need to compute $\rho_N \approx \lambda_n \v_N^\top \y$ in equation (34), without knowledge of the groun truth signal $\x^o$. 
This is clarified in the revised manuscript. 
%Specifically, following 

\vspace{0.2in}
\noindent\textbf{Response 9b:}
Modeling $\lambda_i$'s as an exponential function assumes only the distribution of eigenvalues (graph frequencies) for the underlying graph, NOT the graph signal. 
Specifically, it does not imply a signal residing on the graph kernel is either low-pass or high-pass.


\vspace{\resafter}



{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 10:}
Response 21: Thanks for adding the section on Manifold graph. However, it still remains vague and unclear. For example, what does roughly uniformly distributed samples on a K-dimensional continuous manifold mean? What is the distribution assumption? What is roughly? Is the definition your own or has it been used earlier, in which case kindly cite some of the relevant literature to help the reader. Also, the two properties that you assume that manifold graph: are they themselves the definition of the manifold graph you desire? 
}\vspace{\comafter}

\noindent\textbf{Response 10:}
Graph is naturally a discrete object, and connecting it to a continuous manifold via the common ``manifold assumption" is shockingly common in the machine learning literature \cite{coifman06,hein06}.
For example, assuming that graph nodes are projected samples chosen randomly from a uniform distribution over a manifold domain, \cite{coifman06} showed that the graph Laplacian matrix converges to the continuous Laplace-Beltrami operator at an estimated rate as the number of points approaches infinity and the distances between points go to zero.
Under the same uniform sampling assumption, \cite{hein06} showed that a graph Laplacian regularization term converges to a continuous penalty functional. 
\textbf{Our notion of manifold graph is no different from these earlier works; our innovation comes from efficiently computing a graph embedding given only a manifold graph, and using the computed latent coordinates to promote planar / PWP signal reconstruction via the proposed GNG Laplacian matrix $\cL$.}

Further, the two assumptions we made for a manifold graph are not unusual in the graph embedding literature and have been made previously in kNN graph for ordinal embedding \cite{Terada2014LocalOE, Cucuringu2015OrdinalEO}.
%i) that if $w_{i,j} > w_{i,k}$, then $d_{i,j} < d_{i,k}$ and ii) that if $(i,j) \in \cE$ and $(i,l) \not\in \cE$, then $d_{i,j} < d_{i,l}$. The two properties we assume here stem from the kNN graph construction from discrete samples in a feature space. 

\vspace{\resafter}



{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 11:}
Detailed response 27, thank you for pointing out the exceedingly common nature of the objective. My comment was merely to point out that people, such as myself, who do not solely work on image quality assessment do not find SSIM as a staple metric to understand it when just simply quoted in abbreviation the passing. Same is the case with PSNR.
}\vspace{\comafter}

\noindent\textbf{Response 11:}
We thank the reviewer for this comment.
PSNR and SSIM are indeed the most common image quality metrics in the image processing literature for well over two decades, and we have made effort to explain this basic fact in our revised TSP manuscript.

\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 12:}
Detailed Response 30: I agree, what indeed is the central thesis of the paper has been fairly unclear. Is it planar graph signals or manifold graphs? or is it the fact that you artificially introduce the need for coordinates which essentially restricts your analysis to a handful of realistic cases, and in the other large set of cases where such an embedding is not available, you in turn estimate them from the given graph?
}\vspace{\comafter}

\noindent\textbf{Response 12:}

After two review rounds, at the risk of appearing redundant, we repeat the main contributions of the paper from the Introduction of the paper for the reviewer's perusal: 

\vspace{0.1in}
\begin{enumerate}
\item For graph nodes endowed with latent space coordinates, we define the higher-order Gradient Graph Laplacian Regularizer (GGLR) for graph signal restoration, which retains its quadratic form and thus ease of computation under specified conditions (Theorem 3).
\item We prove GGLR’s promotion of planar signal reconstruction (Theorem 1)---planar signals are 0-frequencies of PSD GNG Laplacian $\cL$. 
We demonstrate that its signal-dependent variant SDGGLR promotes PWP signal reconstruction.
\item For manifold graphs without coordinates, we propose a fast parameter-free graph embedding method (Algorithm 1) to first obtain latent coordinates for graph nodes via fast eigenvector computation before employing SDGGLR.
\item We derive the MSE-minimizing weight parameter $\mu$ for GGLR in a MAP formulation, trading off bias and variance of the signal estimate (Theorem 4).
\item We demonstrate the efficacy of GGLR in four real-world graph signal restoration applications, outperforming previous graph smoothness priors.
\end{enumerate}

We repeat again that the computed node coordinates form a \textit{graph embedding}, whose pairwise Euclidean distances reflect the corresponding node-to-node network distances in the original graph. 
Blindly calling our graph embedding (or \textit{any} graph embedding) ``artificially introduce", when there is a whole graph embedding topic in the machine learning literature \cite{hamilton17, xu21}, seems very misinformed. 
\textbf{This is particular the case when there exists no linear graph signal prior in the literature, and the reviewer has failed to provide any obvious alternative after two review rounds.}

Studying graphs in a restricted setting is wholly consistent with the \textit{graph signal processing} (GSP) literature; 
it is common to study graphs with only positive edges \cite{pang17}, with or without self-loops \cite{anis16}, balanced signed graphs \cite{yang21}, directed acyclic graphs (DAG) \cite{Dinesh2023ModelingVI}, etc. 
In this paper, we propose a new signal prior GGLR exclusively for manifold graphs, where the manifold assumption on graph is rampant in the GSP literature \cite{Hurtado2022StudyOM, Yang2021GroupWiseHI}, with broad applications as shown in the results section. 

\vspace{\resafter}



{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 13:}
Detailed response 32:
The suggestion was owing to the excellent match of the topic to the specific journal that specializes in the topic of graph signals and is more targeted and of to the audience of interest. Is it not the reviewers right to raise a suggestion?
}\vspace{\comafter}

\noindent\textbf{Response 13:}

%We have confirmed with the TSP EiC that 
In the published SPS reviewer guidelines\footnote{https://signalprocessingsociety.org/publications-resources/guidelines-reviewers}, it is stated that
\vspace{0.1in}
\begin{quote}
There are two criteria necessary for a recommendation of acceptance for publication: NOVELTY (new or innovative methods or approaches to a problem of engineering, science, or mathematics) and 
APPROPRIATENESS (\textbf{a complete, well-written manuscript that falls within the scope of the transactions to which it was submitted}).
\end{quote}
It is clear from the second criterion that a reviewer's task is to determine whether a paper is within scope for a journal or conference.
Given a paper is within scope, a paper cannot be rejected because a reviewer personally deems the paper is ``more suitable" to another journal or conference. 
%This point should be obvious to any reviewer.
For example, should a paper on image compression submitted to IEEE International Conference on Image Processing (ICIP), which is clearly within scope of the conference, be rejected solely because a reviewer subjectively deems the paper is ``more suitable" to a more narrowly scoped conference such as Picture Coding Symposium (PCS)? 
Or should a paper on speech recognition submitted to IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP), which is within scope, be rejected because the reviewer thinks the paper is ``more suitable" to more narrowly scoped conference INTERSPEECH?
Clearly, this is not a valid reason to reject the paper, nor the intent of the organized conferences.

Thus, following the published guidelines, we humbly ask the reviewer to comment only on the technical merrits of our submitted manuscript \textit{and} whether our paper is within TSP scope. 

\vspace{\resafter}



{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 14:}
Typo: VBC or this graph on page 15 — should be VBC for this graph?

Also, why is PSNR a meaningful metric for the FIFA and Age estimation datasets over relative mean square error, given that it is not a visual dataset/image dataset?

Overall, the manuscript reads much better now. However, as pointed above, there needs to be more clarity on certain key aspects, particularly in terms of definition and motivation.
}\vspace{\comafter}

\noindent\textbf{Response 14:}
The typo in ``VBC of this graph" is fixed. Thank you for pointing it out.

We first note that peak signal-to-noise ratio (PSNR) is an inverse function of mean square error (MSE)\footnote{https://en.wikipedia.org/wiki/Peak\_signal-to-noise\_ratio}:
\begin{align}
\text{PSNR} = 20 \log_{10} \left(
\frac{\text{MAX}_I^2}{MSE}
\right)
\end{align}
where $\text{MAX}_I$ is the maximum value a sample can take on. 
Thus, a higher PSNR must necessarily mean a smaller MSE, and we do not see a difference presenting PSNR instead of MSE.

For thoroughness, for the FIFA and age estimation datasets, beyond PSNR we also added another metric \textit{accuracy} (Acc) for comparison: accuracy is the number of correct predictions divided by the total number of predictions. Quantitative results in PSNR and accuracy are shown in Table VI of the revised manuscript.

\vspace{\resafter}

==> 2nd-response2reviewers/reviewer_AE.tex <==
{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment:}

``With all due respect, it seems that the authors are confused by the mathematical terminology. Namely, different results used in ANY paper can be called Facts / Claims / Propositions / Lemmas (Lemmata) and, finally, Theorems. These terms all refer to TRUE and (maybe) IMPORTANT results but they play different roles. Namely, any result that is called a Theorem without name of person like Stokes' Theorem or citation is by default claimed to be proven by the authors and to be the main or one on the main contributions of the article. If the authors claim that Theorem 1 is the main result and it has never been known before then the paper must be rejected. This result is definitely known. The authors might look it up in any basic Linear Algebra course. However, if the authors just want to mention it and use as an auxiliary result, they have to call it a Fact/Property/Lemma. For example, Schur's Lemma is an extremely important and even central result in representation theory but everybody calls it lemma. From here we see that being a lemma doesn't mean the result is unimportant.''

I think the critique is justified. The proof has two parts. The first part is indeed a standard result: the graph Laplacian is PSD, and conjugation of a PSD matrix gives a PSD matrix. The second part "GGLR Pr$(\alpha)$ in (22) promotes planar signal reconstruction" is not a proper mathematical statement since "promotes" is a loose term without a proper definition. My suggestion is to separate this into two parts; cite the first part as a Proposition/Lemma and cite a book/paper where this can be found; finally, bring in the second part as a separate remark (or alternatively give a proper mathematical statement that does not rely on ``promotes...'').   
 
}\vspace{\comafter}

\noindent\textbf{Response:}
We thank the AE for the summary comments.
For the first part of Theorem 1, we have added a reference to a standard linear algebra book by Golub and Van Loan \cite{Golub2013MatrixC}. 
For the second part of Theorem 1, we have already provided a definition of ``promote" in footnote 1 in the previous version. 
In this revised version, we further clarified this terminology in the same footnote 1 as:
\vspace{0.1in}
\begin{quote}
By ``promote", we mean adding a non-negative signal prior $\text{Pr}(\x)$ to a minimization objective $f(\x)$ to bias the solution $\x$ where $\text{Pr}(\x) = 0$. See [13] for a comprehensive overview on bias-variance tradeoffs.
\end{quote}
Similarly argued in our response to the AE in the previous review round, we stress here again that \textit{bias-variance tradeoff} is a very well studied topic in machine learning / signal processing literature \cite{Belkin2018ReconcilingMM}.
Saying ``promote" and ``bias" in the context of a minimization problem is not a ``proper mathematical statement" is entirely inconsistent with existing literature \cite{yankelevsky16}, \cite{mahmood18}, \cite{liu19depth}, \cite{cheung21}.

To further clarify what we mean by ``promote" in the special case when the prior is our proposed GGLR, we reworded Theorem 1 as:
\vspace{0.1in}
\begin{quote}
Gradient-induced nodal graph (GNG) Laplacian
$\cL$ is PSD with all planar signals as the $0$-frequencies, and thus GGLR $\x^\top \cL \x$ in (22) promotes planar signal reconstruction,
\ie, planar signals $\x$ compute to $\x^\top \cL \x = 0$.    
\end{quote}
In our specific case, ``promote" here means biasing the solution towards planar signals that are $0$-frequencies of the GNG Laplacian matrix $\cL$. 
We sincerely hope that these revisions are up to the AE's personal standard of mathematical precision. 

\vspace{0.1in}
Lastly, we humbly ask the AE to read not only the reviewers' comments, but our arduously composed responses to the reviewers carefully and thoroughly also before rendering an editorial decision.
We thank the AE for his/her tremendous effort throughout the multiple review rounds.

\vspace{\resafter}




==> GGLR.tex <==
\begin{figure}[t]
\begin{center}
   \includegraphics[width=0.95\linewidth]{fig/3nodeGraph.png}
   %\hspace{0.05in}
   %\includegraphics[width=0.56\linewidth]{long version/fig/4nodeGraph.png}
\end{center}
\vspace{-0.4in}
\caption{Examples of a 3-node graph $\cG$ in (a), the corresponding DAG $\cG^1$ (b), gradient graph $\bar{\cG}^1$ in (c), and resulting GNG $\cH^1$ (d).} 
\label{fig:gradGraphEx}
\end{figure}


We first derive the new graph smoothness prior, \textit{gradient graph Laplacian regularizer} (GGLR), for signal restoration for the case when each graph node is endowed with a low-dimensional latent space coordinate. 
We consider the case when the input manifold graph provides no latent coordinates \textit{a priori} in Section\;\ref{sec:general}.
\blue{We will return to the question of why a manifold graph is necessary in Section\;XXX.}
See Table\;\ref{tab:notations} for notations.


\begin{table}[t!]
\caption{Notations in GGLR Derivation %\blue{from Xue: I guess it's $\cG(\cV, \cE, \W)$ in the first row?}
}
\centering
\begin{scriptsize}
\begin{tabular}{|c|c|} \hline 
$\cG(\cV, \cE, \W)$ & graph with nodes $\cV$, edges $\cE$, adjacency matrix $\W$\\
$\p_i$ & $K$-dimensional coordinate for node $i$ \\
$\F^k$ & gradient operator for dimension $k$ \\
$\cG^k(\cV,\cE^k,\W^k)$ & DAG with nodes $\cV$, edges $\cE^k$, adjacency matrix $\W^k$ \\
$D^k_i$ & out-degree of node $i$ in $\cG^k$ \\
$\g^k$ & $k$-th gradient of signal $\x$ \\
$\bar{\cG}(\bar{\cV}, \bar{\cE}, \V)$ & gradient graph with nodes $\bar{\cV}$, edges $\bar{\cE}$, adjacency matrix $\V$ \\
$\bar{\L}^k$ & gradient graph Laplacian matrix \\
$\cH^k(\cV, \cE^*, \U)$ & gradient-induced nodal graph (GNG) \\
$\L^k$ & GNG Laplacian matrix \\ \hline
\end{tabular}
\end{scriptsize}
\label{tab:notations}
\end{table}


\subsection{Gradient Operator}

Given an undirected graph $\cG = (\cV, \cE, \W)$ with $|\cV| = N$ nodes, we assume here that each node $i \in \{1, \ldots, N\}$ is endowed with a coordinate vector $\p_i \in \mathbb{R}^K$ in $K$-dimensional latent space, where $K \ll N$.
Examples of such graphs include kNN graphs constructed for 2D images or 3D point clouds, where the node coordinates are the sample locations in Euclidean space \cite{hu15,hu15spl,pang17,liu17,dinesh20,dinesh20icip}. 

\blue{For each node $i \in \cV$, we define a \textit{gradient operator} $\F_i \in \mathbb{R}^{K \times N}$ given graph signal $\x \in \mathbb{R}^N$ as follows.
First, define a \textit{directed acyclic graph} (DAG) $\cG^d(\cV,\cE^d,\W^d)$, where directed edges $[i,j] \in \cE^d$ are drawn following the procedure below.
}

\vspace{0.05in}
\noindent
\blue{
\textbf{DAG Construction Procedure}: 
\begin{enumerate}
\item Choose a coordinate $k^*$ from $\{1, \ldots, K\}$.
\item Denote by $\cV_{k^*}$ the set of $N-K$ nodes $i$ in $\cV$ with the smallest $p_{i,k^*}$. 
\item For each node $i \in \cV_{k^*}$, construct $K$ directed edges from $i$ as follows.
\begin{enumerate}[(i)]
\item Add and order 1-hop neighbors $j$ of node $i$ satisfying $p_{j,k^*} > p_{i,k^*}$ by distance to $i$ to list $\cS$.
\item Add directed edge $[i,j^*]$ for closest node $j^*$ to $i$ in list $\cS$. Remove $j^*$ from list $\cS$.
\item Add and order 1-hop neighbors $j$ of node $j^*$ satisfying $p_{j,k^*} > p_{i,k^*}$ to $i$ to list $\cS$.
\item If number of edges $[i,j]$ from node $i$ is $< K$ and $\cS \neq \emptyset$, go to step (ii). 
\end{enumerate}
\end{enumerate}
}

\vspace{0.1in}
\blue{
Using the two properties of a manifold graph in Section\;\ref{subsubsec:manifold}, one can prove the optimality of constructing directed edges $[i,j]$ for each node $i \in \cV_{k^*}$.  
\begin{lemma}
For each node $i \in \cV_{k^*}$, the DAG construction procedure finds the closest $K$ nodes $j$ to node $i$ satisfying $p_{j,k^*} > p_{i,k^*}$.
\end{lemma} 
See Appendix\;\red{XXX} for a proof. 
}

\vspace{0.05in}
\noindent
\blue{
\textbf{Remarks}:
Given node set $\cV_{k^*}$ contains $N-K$ nodes with the smallest $p_{i,k^*}$, 
every node $i \in \cV_{k^*}$ has at least $K$ nodes $j$ satisfying $p_{j,k^*} \geq p_{i,k^*}$.
The condition $p_{j,k^*} > p_{i,k^*}$ is used instead to ensure each directed edge $[i,j]$ satisfies $p_{j,k^*} > p_{i,k^*}$, and thus the constructed directed graph $\cG^d$ contains no cycles. 
This ensures that each manifold gradient computed at each node $i \in \cV_{k^*}$ is distinct. 
For each node $i$ with fewer than $K$ directed edges $[i,j]$ drawn, manifold gradient $\balpha_i$ would not be computed \red{would this work?}.
%DAG is needed to impose ``directionality" when computing gradients on graph $\cG$.
}

%Further, we make the following assumption for simplicity.

%\vspace{0.05in}
%\noindent 
%\textbf{Assumption}:
%Exactly one node (say node $N$) is a \textit{sink}---a node with no outgoing edge---in DAG $\cG^k$. 
%\vspace{0.05in}

%For a manifold graph $\cG$, the assumption is typically satisfied, assuming that a graph is a collection of uniform samples on a convex sampling region in $K$-dimensional latent space (see Fig.\;\ref{fig:finite_graph2} for an illustration). If there are more than one sink in $\cG^k$, we identify a \textit{terminal node} $i^* = \arg \max_i p_{i,k}$, and draw directed edges from other sinks to terminal node $i^*$ to create a unique sink at $i^*$.

\begin{figure}
\centering
\includegraphics[width=2.8in]{fig/finite_graph2.pdf}
\vspace{-0.1in}
\caption{\small Illustration of a finite graph as uniform samples on a convex region of a smooth continuous manifold. 
Boundary nodes (in yellow) have smaller degrees than interior nodes (in blue).
Nodes are mapped into a $K$-dimensional latent vector space.}
\label{fig:finite_graph2}
\vspace{-0.1in}
\end{figure}

\blue{
Denote by $\cE^d(i,k)$ the designation node of the $k$-th directed edge stemming from node $i$ in $\cG^d$.
Given DAG $\cG^d$, we can define entries $\F^i \in \mathbb{R}^{K \times N}$ as
%\begin{align}
%F^k_{i,j} &= \left\{ \begin{array}{ll}
%1 & \mbox{if}~ i=j \\
%-w_{i,j}/D^k_i & \mbox{if}~ [i,j] \in \cE^k \\
%0 & \mbox{o.w.}     
%\end{array} \right. ,
%\label{eq:gradOp}
%\end{align}
\begin{align}
F^i_{m,n} &= \left\{ \begin{array}{ll}
1 & \mbox{if}~ n = i \\
-1 & \mbox{if}~ n = \cE^d(i,m) \\
0 & \mbox{o.w.}
\end{array} \right. 
\end{align}
%where $w_{i,j}$ is weight of edge $(i,j) \in \cE$ in original graph $\cG$, and $D^k_i = \sum_{j\,|\,[i,j] \in \cE^k} w_{i,j}$ is the \textit{out-degree} of node $i$ in $\cG^k$. Definition \eqref{eq:gradOp} ensures that the sum of outgoing edge weights is $-1$ for each node $i$. 
Accompanying $\F^i$ is a coefficient matrix $\C^i \in \mathbb{R}^{K \times K}$ defined as
\begin{align}
C^i_{m,n} = 
p_{i,n} - p_{\cE^d(i,m),n} .
\end{align}
Given input signal $\x \in \mathbb{R}^N$, the hyperplane parameters $\balpha^i = [\alpha_1, \ldots, \alpha_K]^\top$ for node $i \in \cV_{k^*}$ are computed as 
\begin{align}
\balpha^i = (\C^i)^{-1} \F^i \x
\end{align}
}

As an example, consider a $3$-node line graph, shown in Fig.\;\ref{fig:gradGraphEx}(a), where the 1D coordinates for the three nodes are, respectively, $\p_1 = (1)$, $\p_2 = (2)$, and $\p_3 = (3)$. 
The corresponding DAG $\cG^1$ is shown in Fig.\;\ref{fig:gradGraphEx}(b). 
Given $\cG^d$, the corresponding gradient operator $\F^1 \in \mathbb{R}^{2 \times 3}$ is
\begin{align}
\F^1 = \left[ \begin{array}{ccc}
1 & - 1 & 0 \\
0 & 1 & -1
\label{eq:ex_F}
\end{array} \right] .
\end{align}

\subsubsection{Properties of Gradient Operator}

Gradient operator $\F^k$ has the following important properties, which we state formally as a lemma.

\begin{lemma}
A gradient operator $\F^k$ defined in \eqref{eq:gradOp} satisfies the following properties:
\begin{align}
\F^k \,\1 &= \0
\label{eq:grad1} \\
\text{rank}(\F^k) &= N-1
\label{eq:grad2} .
\end{align}
\end{lemma}

\begin{proof}
\eqref{eq:grad1} follows from definition \eqref{eq:gradOp}; for each entry $i$ of $\F^k \1$, we write
\begin{align*}
\left( \F^k \1 \right)_i &= \sum_j F^k_{i,j} = 1 + \sum_{j\neq i} F^k_{i,j} \\
&= 1 - \frac{1}{D^k_i} \sum_{j \,|\,[i,j] \in \cE^k} w_{i,j} = 1 - \frac{D^k_i}{D^k_i} = 0 .
\end{align*}
Since $\left(\F^k \1\right)_i = 0, \forall i$, we conclude that $\F^k \1 = \0$.

Because $\cG^k$ is a DAG, nodes can be renumbered via \textit{topological sorting} \cite{clr} so that if $[i,j] \in \cE^k$, then $i<j$. 
After renumbering, the corresponding matrix $\F^k$ defined in \eqref{eq:gradOp} is in \textit{row echelon form} \cite{strang15}: the leading (non-zero) coefficient of each row $i$---$1$ at entry $(i,i)$ of $\F^k$---is to the right of the row above.
This is true for all $N-1$ rows corresponding to $N-1$ non-sink nodes. 
We can thus conclude that $\text{rank}(\F^k) = N-1$.
\end{proof}

\noindent
\textbf{Remarks}: 
\eqref{eq:grad1} states that the constant signal $\1$ has zero gradient. 
Further, \eqref{eq:grad1} implies that $\F^k(\x + c \1) = \F^k \x, \forall \x \in \mathbb{R}^N, c \in \mathbb{R}$, \ie, gradient operator $\F^k$ is invariant to any constant shift on signal $\x$.
\eqref{eq:grad1} also means that any constant vector is in the \textit{null space} of $\F^k$. 
Recall that the dimensions of null space and \textit{row space} of a $(N-1) \times N$ matrix add up to $N$ \cite{strang15}. 
Given \eqref{eq:grad2}, the dimension of the row space of $\F^k$ is $N-1$. 
See \eqref{eq:ex_F} for an example of $\F^k$ in row echelon form.


\subsection{Gradient Graph}

Given gradient operator $\F^k \in \mathbb{R}^{(N-1) \times N}$ defined w.r.t. the $k$-th latent coordinate, one can compute gradient $\g^k \in \mathbb{R}^{N-1}$ from signal $\x \in \mathbb{R}^N$ as
\begin{align}
\g^k = \F^k \x .
\label{eq:grad}
\end{align}

Given computed gradient $\g^k$ and DAG $\cG^k$, we next construct an undirected \textit{gradient graph} $\bar{\cG}^k(\bar{\cV},\bar{\cE},\V)$: 
for each pair of connected non-sink nodes $i$ and $j$ in $\cG^k$, we connect them in $\bar{\cG}^k$ with an undirected edge with \textit{positive} weight $v_{i,j}^k \in \mathbb{R}^+$.
This construction means graph $\bar{\cG}^k$ has nodes $\bar{\cV} = \cV \setminus \{N\}$ and edges $\bar{\cE} = \cE \setminus \{(i,N)\}_{\forall i}$. 

To promote planar signal reconstruction, we set $v_{i,j}^k = 1$.
Alternatively, one can define $v_{i,j}^k$ in a \textit{signal-dependent} manner as a function of gradients $g^k_i$ and $g^k_j$, \ie, 
\begin{align}
v_{i,j}^k = \exp \left( -
\frac{(g^k_i - g^k_j)^2}{\sigma_g^2}
\right) .
\label{eq:gradWeight}
\end{align}
Note again that $v^k_{i,j} \geq 0$.
\eqref{eq:gradWeight} promotes \textit{piecewise planar} (PWP) signal reconstruction; we discuss PWP in Section\;\ref{subsec:PWP}. 

See Fig.\;\ref{fig:gradGraphEx}(c) for the gradient graph $\bar{\cG}^1$ corresponding to the 3-node DAG $\cG^1$. 
Using $\bar{\cG}^k$, one can define a PSD \textit{gradient graph Laplacian matrix} $\bar{\L}^k$ using definitions in Section\;\ref{sec:prelim}. 
Continuing our 3-node line graph example, the gradient graph Laplacian $\bar{\L}^1$ in this case is
\begin{align}
\bar{\L}^1 = \left[ \begin{array}{cc}
1 & -1 \\
-1 & 1
\end{array} \right] \succeq 0 .
\end{align}


\subsection{Gradient Graph Laplacian Regularizer}

We can now define GGLR $\text{Pr}(\g^k)$ for $\g^k$ as follows:
\begin{align}
\text{Pr}(\g^k) &= \left( \g^k \right)^{\top} \bar{\L}^k \g^k = \left( \F^k \x \right)^{\top} \bar{\L}^k \F^k \x 
\label{eq:GGLR} \\
&= \x^{\top} \underbrace{\left(\F^k \right)^{\top} \bar{\L}^k \F^k}_{\L^k} \x 
= \x^{\top} \L^k \x ,
\end{align}
where $\L^k$ is a graph Laplacian matrix corresponding to a \textit{gradient-induced nodal graph} (GNG) $\cH^k$ computed from $\bar{\L}^k$ and $\F^k$.
Continuing our example, GNG $\cH^1$ for our 3-node line graph is shown in Fig.\;\ref{fig:gradGraphEx}(d), with corresponding GNG Laplacian $\L^1$ computed as
\begin{align}
\L^1 = (\F^1)^{\top} \bar{\L}^1 \F^1 = \left[ \begin{array}{ccc}
1 & -2 & 1  \\
-2 & 4 & -2 \\
1 & -2 & 1
\end{array} \right] .
\end{align}

We see that $\cH^1$ is a 3-node graph with positive edges $w_{1,2} = w_{2,3} = 2$ connecting node pairs $(1,2)$ and $(2,3)$ respectively, and negative edge $w_{1,3} = -1$ connecting node pair $(1,3)$. 
There are no self-loops. 
$\cH^1$ is a \textit{signed} graph with both positive and negative edges.
Despite the presence of a negative edge, $\L^1 = (\F^1)^{\top} \bar{\L}^1 \F^1$ is provably PSD.

\begin{theorem}
Graph Laplacian $\L^k$ corresponding to a gradient-induced nodal graph (GNG) $\cG^k$ is PSD.
\label{thm:GGLR}
\end{theorem}

\begin{proof}
By definition, $\L^k = \left( \F^k \right)^\top \bar{\L}^k \F^k$, where $\bar{\L}^k$ is a graph Laplacian matrix corresponding to a positive graph, and thus is provably PSD \cite{cheung18}.  
We can hence eigen-decompose $\bar{\L}^k$ into $\bar{\L}^k = \U \bSigma \U^\top$, where $\bSigma = \text{diag}(\{\lambda_i\})$ is a diagonal matrix of non-negative eigenvalues $\lambda_i \geq 0, \forall i$. 
Thus, 
\begin{align*}
\x^\top \L^k \x  &= \x^\top \left( \F^k \right)^\top \U \text{diag}(\{\lambda_i\}) \U^{\top} \F^k \x \\
&\stackrel{(a)}{=} \y^\top \text{diag}(\{\lambda_i\}) \y  
= \sum_i \lambda_i y_i^2 \geq 0
\end{align*}
where in $(a)$ we define $\y = \U^\top \F^k \x$.
Since this is true $\forall \x$, $\L^k$ is PSD. 
\end{proof}

\noindent
\textbf{Remarks}:
Signed graphs were studied previously in several GSP works. 
\cite{su17} studied GFT for signed graphs, where each endpoint of an edge $(i,j)$ with negative weight $w_{i,j} < 0$ has a self-loop with weight $2|w_{i,j}|$ to ensure the resulting graph Laplacian is PSD. 
Orthogonally, to ensure PSDness, \cite{cheung18tsipn} shifted up the spectrum of Laplacian $\L$ by computing $\L + |\lambda_{\min}^-|\, \I$, where $\lambda_{\min}^-$ is a lower bound of the smallest (negative) eigenvalue of $\L$.
\cite{yang21} studied the special case of \textit{balanced} signed graphs (graphs with no cycle of odd number of negative edges).
In contrast, a GNG---as shown in Fig.\;\ref{fig:gradGraphEx}(d)---has no self-loops and is not balanced in general, yet its corresponding GNG Laplacian is provably PSD.
We study the spectral properties of GNG Laplacians next.


\subsection{Spectral Properties of GNG Laplacian}

We state the following important spectral property of a GNG Laplacian formally.

\begin{theorem}
GNG Laplacian $\L^k$ for GNG $\cH^k$ has \textit{two} eigenvectors $\u_1$ and $\u_2$ corresponding to eigenvalue $0$. 
\label{thm:GGLR2}
\end{theorem}

\begin{proof}
The first (unnormalized) eigenvector $\u_1$ is $\1$, stemming from the first property \eqref{eq:grad1} of the gradient operator $\F^k$.
Specifically,
\begin{align}
\L^k \1 &= ( \F^k )^{\top} \bar{\L}^k \F^k \1 \\
&= ( \F^k )^{\top} \bar{\L}^k \0 = \0 .
\end{align}

The second eigenvector $\u_2$ can be derived from the first (unnormalized) eigenvector $\1$ of gradient graph Laplacian $\bar{\L}^k$ corresponding to eigenvalue $0$ and the second property \eqref{eq:grad2} of the gradient operator $\F^k$.
Specifically,
\begin{align}
\L^k \u_2 &= ( \F^k )^{\top} \bar{\L}^k \F^k \u_2 = \0, ~~\mbox{if}~ \F^k \u_2 = \1 \\
\therefore \u_2 &= \left(\F^k \right)^+ \1 = (\F^k)^{\top} \left( \F^k (\F^k)^{\top} \right)^{-1} \1
\end{align}
where $(\F^k)^+$ is the \textit{right pseudo-inverse} of matrix $\F^k$.
This means that $\F^k \u_2 = \F^k (\F^k)^+ \1 = \1$, and thus $\L^k \u_2 = \0$. 
Note that the inverse of $(N-1) \times (N-1)$ matrix $\F^k (\F^k)^{\top}$ exists since $\F^k$ is full row-rank due to \eqref{eq:grad2}. 
\end{proof}

\noindent
\textbf{Remark}: 
Given Theorem\;\ref{thm:GGLR2}, one can see that multiplying $\L^k$ by any linear combination $\v = \alpha_1 \u_1 + \alpha_2 \u_2$ of the first two eigenvectors $\u_1$ and $\u_2$ (corresponding to eigenvalue $0$) will also result in $\0$. 
Following our 3-node line graph example, $\u_2 = [1 ~0 ~-1]^{\top}$. 
Assuming $\alpha_1 = 1$ and $\alpha_2 = \alpha$ for simplicity, $\v = [1 + \alpha ~~ 1 ~~ 1 - \alpha]^{\top}$, which is a line with slope $-\alpha$. 
This agrees with our intuition that GGLR promoting planar signal reconstruction should evaluate to $0$ for any linear signal on a line graph. 


\subsection{Piecewise Planar Signal Reconstruction}
\label{subsec:PWP}

Unlike SDGLR in \cite{pang17,liu17} that promotes PWC signal reconstruction, minimizing signal-dependent GGLR (SDGGLR) promotes PWP signal reconstruction.
We demonstrate this behavior by extending our analysis for SDGLR in Section\;\ref{subsec:defn}. 

First, define \textit{square difference of gradient} $\delta^k_{i,j} \triangleq (g^k_i - g^k_j)^2$.
Signal-dependent edge weight $v^k_{i,j}$ for gradient graph $\bar{\cG}^k$ is thus $v^k_{i,j} = \exp \left( - \delta^k_{i,j} / \sigma_g^2 \right)$. 
Writing GGLR \eqref{eq:GGLR} as a sum
\begin{align}
\left( \g^k \right)^\top \bar{\L}^k \g^k &= \sum_{(i,j) \in \bar{\cE}^k} \exp \left( - \frac{\delta^k_{i,j}}{\sigma_g^2}\right) \delta^k_{i,j}, 
\end{align}
we see that each term in the sum corresponding to $(i,j) \in \bar{\cE}^k$ goes to $0$ if either i) $\delta^k_{i,j} \approx 0$, or ii) $\delta^k_{i,j} \approx \infty$ (in which case edge weight $v^k_{i,j} \approx 0$). 
Thus, minimizing GGLR \eqref{eq:GGLR} iteratively would converge to a solution $\x^*$ where clusters of connected node-pairs in $\bar{\cG}^k$ have very small $\delta^k_{i,j}$, while connected node-pairs across clusters have very large $\delta^k_{i,j}$. 

As an illustrative example, consider a 5-node line graph $\cG^1$ with initial noisy signal $\y = [2 ~2.8 ~3.1 ~2.5 ~1.2]^\top$.
Setting $\sigma_g^2 = 0.5$, the corresponding gradient graph $\bar{\cG}^1$ and GNG are shown in Fig.\;\ref{fig:gradient_graph}(a) and (b), respectively. 
Using an iterative algorithm that alternately computes a signal by minimizing objective $\min_{\x} \|\y-\x\|^2_2 + \mu \x^\top \L^1 \x$ and updates edge weights $v^1_{i,j} = \exp \left( - \delta^1_{i,j} / \sigma_g^2 \right)$ in $\bar{\L}^1$, where $\mu = 0.25$, it converges to solution $\x^* = [2.08 ~ 2.66 ~3.25 ~2.29 ~1.32]$ after $6$ iterations. 
The corresponding gradient graph and GNG are shown in Fig.\;\ref{fig:gradient_graph}(c) and (d), respectively.
In Fig.\;\ref{fig:gradient_graph}(f), we see that samples of the converged signal in the nodal domain follows two straight lines. 
In Fig.\;\ref{fig:gradient_graph}(e), we see that neighboring nodes have the same gradients except node $(2,3)$.
The converged signal $\x^*$ that minimizes SDGGLR $\x^\top \L^1(\x) \x =  1.7e-04$ is PWP.

\begin{figure}
\centering
\begin{tabular}{cc}
\includegraphics[width=3.4in]{fig/gradientGraphExample.pdf}
\vspace{-0.05in}
\end{tabular}
\caption{\small (a) An example gradient graph $\bar{\cG}^1$ with edge weights initialized from a noisy $5$-node signal on a line graph. 
(b) A corresponding GNG $\cH^1$ to the gradient graph in (a).
(c) A gradient graph with edge weights converged after $6$ iterations.
(d) A corresponding GNG to the gradient graph in (c). 
(e) Computed gradients $\g^1$'s after different numbers of iterations. 
(f) Computed signals $\x$'s using GLR or GGLR for regularization after different numbers of iterations.}
\label{fig:gradient_graph}
%\vspace{-0.1in}
\end{figure}



%\subsection{Robust Gradient Estimation}

%Computation of edge weights in the gradient graph requires the difference of gradients $g^k_i - g^k_j = x_{i+1} - x_i - x_{j+1} + x_j$. If each sample $x_i$ is corrupted by zero-mean additive noise with variance $\sigma^2$, then variable $\g^k_i - \g^k_j$ suffers from \textit{four times} the noise variance $4\sigma^2$. Hence an accurate estimate of gradient $g^k_i$ is essential. 

%We compute robust estimates of gradients following a procedure in \cite{chao21}. Denote by $f(\x)$ the signal at coordinate $\x$. Via Taylor series, we can write
%\begin{align}
%f(\x) = f(\a) + \nabla f(\a) (\x - \a) + \cO(\|\x - \a\|^2)
%\label{eq:Taylor}
%\end{align}
%where $\nabla f(\a) \in \mathbb{R}^K$ is the gradient of $f(\cdot)$ evaluated at $\a$. Suppose we approximate $f(\x)$ using only the first two terms:
%\begin{align}
%f(\x) \approx f(\a) + \nabla f(\a) (\x - \a) .
%\label{eq:Taylor2}
%\end{align}
%We estimate $\nabla f(\a)$ using $n$ nearest signal samples, $\x^1, \ldots, \x^n$ to coordinate $\a$. Denote by $\R \in \mathbb{R}^n$ the vector of signal difference between $\x^i$'s and $\a$. From \eqref{eq:Taylor2}, we can write
%\begin{align}
%\R = \X \cdot \nabla f(\a) = 
%\left[ \begin{array}{c}
%f(\x^1) - f(\a) \\
%\vdots \\
%f(\x^n) - f(\a)
%\end{array} \right]
%\end{align}
%where
%\begin{align}
%\X = \left[ \begin{array}{c}
%(\x^1 - \a)^{\top} \\
%\vdots \\
%(\x^n - \a)^{\top}
%\end{array} \right]
%\end{align}
%is a $n \times K$ matrix. The optimal gradient can be computed as
%\begin{align}
%\nabla f(\a)^* = \min_{\nabla f(\a)} \|\R - \X \cdot \nabla f(\a) \|^2_2 .    
%\end{align}
%The closed-form solution is
%\begin{align}
%\nabla f(\a)^* = (\X^{\top} \X)^{-1} \X^\top \R     
%\end{align}
%where $\X^+ = (\X^{\top} \X)^{-1} \X^\top$ is the left pseudo-inverse of $\X$. 


\subsection{MAP Optimization}
\label{subsec:MAP}

We now formulate a \textit{maximum a posteriori} (MAP) optimization problem using a linear signal formation model and GGLR \eqref{eq:GGLR} as signal prior, resulting in
\begin{align}
\min_\x \|\y - \H \x\|^2_2 + \frac{\mu}{K} \sum_{k=1}^K \x^\top \L^k \x
\label{eq:MAP_general}
\end{align}
where $\y \in \mathbb{R}^M$ is an observation vector, $\H \in \mathbb{R}^{M \times N}$, $M \leq N$, is the signal-to-observation mapping matrix, and $\mu >0 $ is a tradeoff parameter (to be discussed in details in Section\;\ref{sec:optPara}). 
For example, $\H$ is an identity matrix if \eqref{eq:MAP_general} is a denoising problem \cite{pang17}, $\H$ is a $0$-$1$ sampling matrix if \eqref{eq:MAP_general} is an interpolation problem \cite{chen21}, and $\H$ is a blur filter if \eqref{eq:MAP_general} is a deblurring problem \cite{bai19}. 
We discuss specific applications of \eqref{eq:MAP_general} in Section\;\ref{sec:results}.

\eqref{eq:MAP_general} has an easily computable solution if $\H$ satisfies two conditions, which we state formally below.

\begin{lemma}
Optimization \eqref{eq:MAP_general} has the following closed-form solution 
\begin{align}
\x^* = { \underbrace{ \left( \H^\top \H + \frac{\mu}{K} \sum_{k=1}^K \L^k \right)}_{\bPhi}  }^{-1} \H^\top \y 
\label{eq:MAP_sol_general}
\end{align}
if $\H$ is full row-rank, and $\exists k^* \in \{1, \ldots, K\}$ such that matrix $\M^{k^*} = [ \H^+ \H \1_N ~~ \H^+ \H (\F^{k^*})^+ \1_{N-1} ] \in \mathbb{R}^{N \times 2}$ has rank 2.
\label{lemma:closedForm}
\end{lemma}
\vspace{0.05in}

See Appendix\;\ref{append:invertible} for a proof.
Note that \eqref{eq:MAP_sol_general} can be solved as a linear system $\bPhi \x^* = \H^\top \y$ efficiently without matrix inverse using CG \cite{axelsson1986rate}.  
Condition requiring $\H$ to be full row-rank means that rows in $\H$ are linearly independent. 
Condition requiring $\M^{k^*}$ to be full column-rank (rank $2$) means that projections of first and second eigenvectors of $\L^{k^*}$, $\1$ and $(\F^{k^*})^+ \1$, onto the row space $\cR(\H)$ of $\H$ are linearly independent.
Both conditions are typically satisfied in practice.
%i) $\H$ for denoising and interpolation is always full row-rank, and ii) first and second eigenvectors of $\L^{k^*}$ are orthogonal by definition, and their projections to row space $\mathcal{R}(\H)$ are 


==> Graph_Const.tex <==
%For inpainting, gradient  is an important feature to preserve  image structures.


\subsection{Horizontal Gradient Graph}

Given an image $\X \in \mathbb{R}^{M\times N}$, we compute its \textit{horizontal gradient} $\G^h \in \mathbb{R}^{M\times (N-1)}$ as the intensity differences between horizontally neighboring pixels, \ie, 
\begin{align}
\G^h_{k,l} = \X_{k,l+1} - \X_{k,l}   
\end{align}
for $1 \leq k \leq M$ and $1 \leq l \leq N-1$. We rewrite $\G^h$ in vector form $\mathbf{g}^h={\rm vec}(\G^h)\in\mathbb{R}^{M(N-1)\times 1}$, where ${\rm vec}(\cdot)$ denotes the vectorization operator stacking columns of a matrix into a vector. We then have a matrix representation $\g^h = \F^h \x$, where $\x={\rm vec}(\X)$ and $\F^h \in \mathbb{R}^{M(N-1) \times MN}$ is the linear horizontal gradient operator.

Next, we define a \textit{horizontal gradient graph} $\cG^h$ consisting of $M(N-1)$ nodes corresponding to elements of $\g^h$. Denote by $\l_i \in \mathbb{R}^2$ and $\g^h_i \in \mathbb{R}$ the gradient's 2D grid location and value for element $i$ in $\g^h$, respectively. 
Similar to \eqref{eq:edgeWeight0}, we define the weight $w^h_{i,j}$ for an edge connecting nodes $i$ and $j$ as

\vspace{-0.1in}
\begin{small}
\begin{align} 
w^h_{i,j}= \left\{ \begin{array}{ll}
\exp\left(- \frac{|\g^h_i - \g^h_j|^2}{\sigma^2}\right) & \|\l_i-\l_j\|_2 \leq \epsilon \\
0 & \mbox{o.w.}  
\end{array}\right.
\label{eq:edgeWeight_h}
\end{align}
\end{small}\noindent
where $\|\l_i-\l_j\|_2$ is the Euclidean distance between gradients  $i$ and $j$. 
Parameter $\epsilon$ controls the size of the local neighborhood, and $\sigma$ is a chosen parameter so that edge weights $w^h_{i,j}$ are well distributed between $0$ and $1$. 
Define next an \textit{adjacency matrix} $\W^h \in \mathbb{R}^{M(N-1) \times M(N-1)}$ where $W^h_{i,j} = w^h_{i,j}$.
A graph $\cG^h$ is completely characterized by the adjacency matrix $\W^h$.


\subsubsection{GGLR for Horizontal Gradients}

We next define the diagonal \textit{degree matrix} $\D^h$ with diagonal elements $\D^h_{i,i} = \sum_j \W^h_{i,j}$. 
We can then define a \textit{graph Laplacian matrix} $\L^h \in \mathbb{R}^{M(N-1) \times M(N-1)}$ as $\L^h = \D^h - \W^h \in \mathbb{R}^{M(N-1)\times M(N-1)}$. 
Given that the edge weights are non-negative, one can show that the real symmetric matrix $\L^h$ is \textit{positive semi-definite} (PSD) via the Gershgorin circle theorem \cite{cheung18}. 
Since edge weights are defined w.r.t. signal $\x$, Laplacian $\L^h(\x)$ is a function of $\x$. 
We now write GLR for gradient $\g^h$
\begin{align} 
\left(\g^h \right)^{\top} \L^h \g^h &= \sum_{i=1}^{M(N-1)} \sum_{j=1}^{M(N-1)} w^h_{i,j} (\g^h_j-\g^h_i)^2 
\label{eq:GGLR_H1} \\
%&= \left( \F^h \x \right)^{\top} \L^h \left( \F^h \x \right) \\
&= \x^{\top} \underbrace{( \F^h )^{\top} \L^h \F^h}_{\cL^h} \x
= \x^{\top} \cL^h \x
\label{eq:GGLR_H}
\end{align}
where $\cL^h$ is also PSD since $\L^h$ is PSD.
Thus GLR for gradient $\g^h$ can also be computed in the pixel domain on $\x$ in quadratic form using matrix $\cL^h$. 
Note that $M+1$ smallest eigenvalues of $\cL^h$ are $0$; $\cL^h$ inherits one zero eigenvalue from Laplacian $\L^h$, and adds $M$ more due to dimension expansion from $M(N-1)$ to $MN$. 
This has important implication when we derive a tradeoff parameter in Section\;\ref{subsec:tradeoff}.
We call \eqref{eq:GGLR_H} the \textit{horizontal GGLR} for signal $\x$.


\subsection{Vertical Gradient Graph}

Similarly, we define the gradient in the vertical direction  $\G^v \in \mathbb{R}^{(M-1)\times N}$ as  $\G^v_{k,l} = \X_{k+1,l} - \X_{k,l}$ for $1 \leq k \leq M-1$ and $1 \leq l \leq N-1$. 
We have a similar matrix representation in the vertical direction $\g^v = \F^v \x$, where  $\F^v \in \mathbb{R}^{(M-1)N \times MN}$ is the vertical gradient operator. 
The \textit{vertical GGLR} is thus $\x^{\top} \cL^v \x$, where $\cL^v = (\F^v)^{\top} \L^v \F^v$. 
$N+1$ smallest eigenvalues of $\cL^v$ are zeros. 

%\red{the problem when computing the difference of gradients is that now u suffer from 4 times the noise variance instead of 2. given in inpainting u don't have accurate estimate of gradients, how is this a good idea?}

%\red{gradient is $g_{ij} = x_i - x_j$, so if each pixel is corrupted by an additive noise with variance $\sigma$, then $g_{ij}$ is corrupted by TWICE the variance. if u now have gradient of gradients $h_{ijst} = g_{ij} - g_{st}$, then obviously u have 4 times the noise variance.} 
%Similarly, the vertical gradient $\mathbf{g}_v$ is assumed smooth with respect to a \textit{vertical gradient graph} $\mathcal{G}_v$ with $(M-1)N$ vertices and weight matix $\mathbf{W}_v$. Corresponding graph Laplacian matrix for $\mathbf{g}_v$ is expressed as $\mathbf{L}_v$.

==> apps.tex <==

We now present a series of experiments in which we test the proposed GGLR. We consider four applications: 2D image interpolation, 3D point cloud color denoising, kNN graph based face classification and social network data interpolation.
\subsection{Image Interpolation} 

Given 2D image $\X$, we compute its \textit{horizontal gradient} $\G^1$ as the intensity differences between horizontally neighboring pixels. We rewrite $\G^1$ in vector form $\mathbf{g}^1={\rm vec}(\G^1)$, where ${\rm vec}(\cdot)$ denotes the vectorization operator stacking columns of a matrix into a vector. 
Thus we have a matrix representation $\g^1 = \F^1 \x$, where $\x={\rm vec}(\X)$ and $\F^1$ is the horizontal gradient operator.

Next, we define a \textit{horizontal gradient graph} $\cG^1$ consisting of nodes corresponding to elements of $\g^1$. 
%Denote by $g^h_i \in \mathbb{R}$ the $i$-th element in $\g^h$. 
Similar to \eqref{eq:edgeWeight0}, we define the weight $w^1_{i,j}$ for an edge connecting nodes $i$ and $j$ as

\vspace{-0.15in}
\begin{small}
\begin{align} 
w^1_{i,j}= \left\{ \begin{array}{ll}
\exp\left(- \frac{|g^1_i - g^1_j|^2}{\sigma_g^2}\right) & j \in \cN_i \\
0 & \mbox{o.w.}  
\end{array}\right.
\label{eq:edgeWeight_img}
\end{align}
\end{small}\noindent
%where $\|\l_i-\l_j\|_2$ is the Euclidean distance between gradients  $i$ and $j$. 
where $\cN_i$ is a defined local neighborhood centered at gradient $i$. 
%Parameter $\epsilon$ controls the size of the local neighborhood, and 
$\sigma_g > 0$ is a chosen parameter so that edge weights $w^1_{i,j}$ are well distributed between $0$ and $1$. 
Define next an \textit{adjacency matrix} $\W^1$ where $W^1_{i,j} = w^1_{i,j}$.
A graph $\cG^1$ is completely characterized by the adjacency matrix $\W^1$. We next define horizontal diagonal degree matrix $\D^1$ and graph Laplacian matrix $\bar{\L}^1=\D^1-\W^1$.

Similarly, we define the gradient in the vertical direction  $\G^2$, and have a matrix representation $\g^2 = \F^2 \x$, where  $\F^2 $ is the vertical gradient operator. The vertical gradient graph Laplacian matrix is thus $\bar{\L}^2$.

The \textit{GGLR} is thus $\x^{\top} (\L^1+ \L^2) \x$, where $\L^1 = (\F^1)^{\top} \bar{\L}^1 \F^1$ and $\L^2 = (\F^2)^{\top} \bar{\L}^2 \F^2$.
Note that $\L^1$ and $\L^2$ are signal-dependent functions of $\x$ due to \eqref{eq:edgeWeight_img}.
As done in \cite{pang17},\cite{liu17} for GLR, we solve \eqref{eq:MAP_sol_general} via an iterative approach.
For fixed $\L^1$ and $\L^2$, we first compute optimal $\x^*$.
We then update edge weights using \eqref{eq:edgeWeight_img} in the two gradient graphs $\cG^1$ and $\cG^2$ having computed gradients $\g^1$ and $\g^2$ from solution $\x^*$.  
We repeat these two steps until convergence. 

%Since $\B$ is symmetric, sparse and PD, \eqref{eq:LS} can be solved efficiently using \textit{conjugate gradient} (CG) \cite{axelsson1986rate}, without computing matrix inverse, in $\cO(cMN)$, where $c$ is the iteration number in CG.

Given a corrupted image $\y$ with dimension $K=2$, we can compute an optimal $\mu$ based on MSE analysis in Section\;\ref{subsec:MAP}. 
The optimization algorithm for SDGGLR is described in Algorithm \ref{alg:alg1}.

\begin{algorithm}[htb]
\caption{ SDGGLR for graph signal interpolation}
\label{alg:alg1}
\begin{algorithmic}[1]
\REQUIRE~~Corrupted signal $\y$, $K$, and selection matrix $\H$. \\
\STATE Initialize $\x=\y$.
\STATE Compute gradient operator $\{\F^{k}\}_{k=1}^{K}$.\\
\WHILE{not converge}
\STATE Compute signal gradient $\{\g^k\}_{k=1}^{K}$.\\
\STATE Compute adjacency matrix $\{\W^k\}_{k=1}^{K}$.\\
\STATE Compute gradient graph Laplacian matrix $\{\bar{\L}^k\}_{k=1}^{K}$.\\
\STATE Estimate the parameter $\mu$ and update $\Phi$.\\
\STATE Update $\x$ by solving \eqref{eq:MAP_sol_general}.
\ENDWHILE
\ENSURE ~~Restored signal $\x$.
\end{algorithmic}
\end{algorithm}

\subsection{3D Point Cloud Color Denoising} 


We define a point cloud as a set of discrete samples of 3D coordinates of an object's 2D surface in 3D space.
For fair comparison, we convert the red, green, and blue values of an RGB point cloud to luminance (Y) and chrominance (Cb and Cr) values of a YCbCr point cloud. Here, we only select luminance values as the signals of point cloud.
Let $\mathbf{d}$ be the luminance vector for the point cloud. Noise-corrupted $\mathbf{d}$ can be simply modeled as $\mathbf{d=c+n}$, where $\mathbf{c}$ is the true  luminance value, $\mathbf{n}$ is the additive noise. The goal is to recover $\mathbf{c}$ given only noise-corrupted observation $\mathbf{d}$.

Different from 2D image, 3D point cloud has no fixed number of equally spaced adjacent points. We construct a $k$-nearest neighbor($k$NN) graph to connect 3D points in a given point cloud based on Euclidean distance in 3D coordinates.
Each 3D point is represented by a node and is connected through edges to its $k$ nearest neighbors. Let $\W$ be the adjacency matrix, the edge weight of point cloud between nodes $i$ and $j$ is computed by:

\begin{small}
\begin{align} 
\W_{i,j}= \left\{ \begin{array}{ll}
\exp\left(- \frac{\|\p_i - \p_j\|^2}{\sigma_p^2_2}- \frac{\|\d_i - \d_j\|^2_2}{\sigma_d^2}\right) & j \in \cN_i \\
0 & \mbox{o.w.}  
\end{array}\right.
\label{eq:edgeWeight_pc}
\end{align}
\end{small}\noindent
where $\cN_i$ is a defined $\kappa$ nearest neighborhood centered at gradient $i$. $\p_i$ is the 3D coordinates of point $i$, and $\sigma_p$ and $\sigma_d$ are two parameters.


\begin{algorithm}[htb]
\caption{ Gradient operator for graph with coordinates}
\label{alg:alg2}
\begin{algorithmic}[1]
\REQUIRE~~Adjacency matrix $\W$ and coordinates $\P\in\mathbb{R}^{K\times N}$. \\
\STATE Initialize gradient operator $\F^k=\I,k=1,\cdots,K$.
\FOR{$i=1:N$}
\FOR{$k=1:K$}
\FOR{$j\in\cN_i$}
\IF{$\P_i^k>\P_j^k$}
%\STATE $\F^k_{i,i}=\frac{1}{\epsilon+\P_i^k-\P_j^k}$\\
\STATE $\F^k_{i,j}=-\W_{i,j}$\\
%\ELSE
%\STATE $\F^k_{j,i}=\F^k_{j,i}-\eta$\\
%\STATE $\F^k_{j,j}=\F^k_{j,j}+\eta$\\
\ENDIF 
\ENDFOR
\STATE Compute node $i$'s out-degree $D_i^k$.
\STATE $\F_{i,j}^k=\F_{i,j}^k/D_i^k$,$\forall j\in\cN_i$
\ENDFOR
\ENDFOR
\ENSURE ~~Gradient operator $\F^k,k=1,\cdots,K$.
\end{algorithmic}
\end{algorithm}



We compute the gradient operator $\F^k$ in $K$-dimensional directions, as shown in Algorithm \ref{alg:alg2}. The weight of the edge on $k$-th gradient graph between nodes $i$ and $j$ is computed by:

\begin{small}
\begin{align} 
w^k_{i,j}= \left\{ \begin{array}{ll}
\exp\left(- \frac{|g^k_i - g^k_j|^2}{\sigma_g^2}\right) & j \in \cN_i \\
0 & \mbox{o.w.}  
\end{array}\right.
\label{eq:edgeWeight_pc2}
\end{align}
\end{small}\noindent
%where $\cN_i^k$ is a defined $\kappa$ nearest neighborhood centered at gradient $i$. 
We consider denoising corresponding to $\H=\I$ in (\ref{eq:MAP_general}). The GGLR based point cloud color denoising can be formulated as an unconstrained problem
\begin{equation}
    \min_{\mathbf{c}}\|\mathbf{d}-\mathbf{c}\|_2^2+\frac{\mu}{3} \mathbf{c}^{\top}(\mathbf{L}^1+\mathbf{L}^2+\mathbf{L}^3)\mathbf{c}
\end{equation}

The optimization algorithm of point cloud color denoising is similar to Algorithm \ref{alg:alg1}.

\subsection{Face Classification and Social Network Data Interpolation}


We evaluate the proposed GGLR for graphs without coordinates. The first type of test datasets are $k$-nearest neighbor ($k$NN) graphs. Since face datasets have a known low-dimensional manifold structure, three kNN graphs were constructed from dataset JAFFE\cite{JAFFE}, AT\&T \cite{ATT}, and Extended YaleB \cite{Georghiades2001EYB} based on Euclidean distances between facial image features. 
The faces are represented by an 20-nearest neighbor graph, in which nodes represent face images, and each node is connected to 20 other nodes that represent the most similar faces. The description of datasets is shown in Table \ref{tab:dataset}.

For a graph with unknown construction, we use VBC discussed in Section to evaluate its quality as a manifold graph. As shown in Table \ref{tab:vbc}, kNN graphs have relatively small VBCs and thus are better manifold graphs than citation networks.
We consider a semi-supervised face classification problem, that is, classification with some labeled data and the remaining unlabeled data. The task is to classify the unlabeled faces given a graph without coordinates. We randomly labeled 1\%, 10\%, 30\%, 50\%, 70\% and 90\% nodes, called the \textit{labeling ratio}. 
We then applied the graph signal interpolation to estimate the labels for the remaining nodes.

\begin{table}   
\begin{center}   
\caption{Description of datasets}  
\label{tab:dataset} 
\begin{footnotesize}
\begin{tabular}{|c|c|c|c|c|}   
\hline   Dataset & $|\cV|$ & $|\cE|$ & $K$& $Clusters$  \\   
\hline   JAFFE & 200 & 1822  & 2 & 10  \\ 
\hline   AT\&T & 400 & 2054  & 2& 40\\  
\hline   EYB & 2414 & 32375& 2 & 38 \\   
%\hline   AR& 2600  & 34262 & 2& 100  \\  
%\hline   Karate& 34  &154  & 2& 2  \\ 
\hline   Football& 105  &613  & 2& 12  \\ 
\hline   LastFM& 882  &1597  & 2& 18  \\
\hline   
\end{tabular}   
\end{footnotesize}
\end{center}   
\end{table}


 The graph signal here is the label assigned to the faces. For kNN graph without coordinates, we first apply the proposed graph embedding to obtain coordinates. The steps are summarized in Algorithm \ref{alg:alg3}.

\begin{algorithm}[htb]
\caption{ Embedding for graph without coordinates}
\label{alg:alg3}
\begin{algorithmic}[1]
\REQUIRE~~Adjacency matrix $\W$ and dimension $K$. \\
\STATE Compute $\L$ and two-hop matrix $\Q$. \\
\STATE Compute $\epsilon=\lambda_{\min}^{(2)}(\Q)$.\\ 
\STATE Compute $\mu$ by solving (39).\\
\STATE Compute $\A=\L-\mu\Q+\epsilon\I$ and diagonal matrix $\B$.\\
\STATE Computing the first $K+1$ generalized eigen-pair for matrix pair $(\A, \B)$, and let $\P$ be the eigenvector matrix corresponding to the 2nd to $K+1$st smallest eigenvalues.\\
\ENSURE ~~Embedding coordinates $\P$.  
\end{algorithmic}
\end{algorithm}

The second type of datasets consists of social networks: Football \cite{Girvan2002football} and LastFM\cite{Rozemberczki2020Lastfm}. The nodes in the Football dataset  are Division IA colleges, the edges represent games in the 2000 regular season, and the labels represent conferences.
A social network of LastFM users which was collected from the public API in March 2020. Nodes are LastFM users from Asian countries and edges are mutual follower relationships between them. The labels represent the location of users. In order to show the PWP of social networks, we select a connected subgraph from dataset Lastfm by removing nodes with degrees smaller than 1. The number of nodes and edges are described in Table \ref{tab:dataset}.

Similarly, we first compute graph embedding to obtain the latent coordinates by Algorithm \ref{alg:alg3}, and then compute gradient operator as done in Algorithm \ref{alg:alg2}, and finally perform signal interpolation by Algorithm \ref{alg:alg1} 

==> embedding.tex <==
%coordinate $\p_i$ of an node $i \in \cU \subset \cV$, where $|\cU| = M$, can be approximately expressed as a linear combination of coordinates $\p_j$ of connected neighboring nodes $j$ in graph $\cG$, \ie,
%\begin{align}
%\p_i \approx \sum_{j \,|\, (i,j) \in \cE} \bar{w}_{i,j} \p_j, ~~~ \forall i \in \cU
%\end{align}
%where $\bar{w}_{i,j} = w_{i,j} / \sum_{l|(i,l) \in \cE} w_{i,l}$ is a normalized version of $w_{i,j}$.

%LLE assumes that the coordinate vectors for the $N$ points, $\q_k = [p_{1,k}, p_{2,k}, \ldots, p_{N,k}]$, $k \in \{1, \ldots, K\}$, are \textit{orthonormal}. This \textit{unit variance} requirement $\q_i^{\top} \q_j = \delta_{i-j}$ ensures two desirable properties: i) $\q_i^{\top} \q_i = 1$ means that the pathological solution $\q_i = \0, \forall i$ is not possible, and ii) $\q_i^{\top} \q_j = 0, \forall i \neq j$ means that coordinate vectors cannot be the same. See Fig.\;\red{add fig} for examples where coordinate vectors do (not) satisfy the orthonormal condition. With the orthonormal requirement, the optimization becomes
%\begin{align}
%\min_{\{\p_i\}} \sum_{i \in \cU} \sum_{j | (i,j) \in \cE} \| \p_i - \bar{w}_{i,j} \p_j \|^2_2, ~~~\mbox{s.t.}~~ \q_i^{\top} \q_j = \delta_{i-j}
%\label{eq:LLE0}
%\end{align}
%where $\delta_{i-j}$ is the discrete Dirac-delta function.


\subsection{Defining Objective}

We first define $\P \in \mathbb{R}^{N \times K}$, where the $i$-th row of $\P$ contains the $K$-dimensional latent vector $\p_i \in \mathbb{R}^K$ for node $i \in \cV$.
For notation convenience, we define also $\q_k$ as the $k$-th column of $\P$---the $k$-th coordinate of all $N$ nodes. 
To minimize the latent space distances between connected $1$-hop neighbors $(i,j) \in \cE$ in original graph $\cG$, we first minimize the GLR \cite{pang17}:
\begin{align}
\min_{\P \,|\, \P^{\top} \P = \I} \text{tr} \left( \P^{\top} \L \P \right) 
&= \sum_{k=1}^K \q_k^{\top} \L \q_k 
\label{eq:obj1} \\
&= \sum_{k=1}^K \sum_{(i,j) \in \cE} w_{i,j} (q_{k,i} - q_{k,j})^2 
\nonumber 
\end{align}
where $q_{k,i}$ is the $k$-th latent coordinate of node $i$.
Like LLE \cite{LLE}, orthogonality condition $\P^{\top} \P = \I$ is added to ensure $\q_i^{\top} \q_j = \delta_{i-j}$. 
Minimizing \eqref{eq:obj1} would minimize the squared Euclidean distance $\|\p_i - \p_j\|^2_2$ between connected node pair $(i,j)$ in the latent space.
This objective thus preserves the \textit{first-order proximity} of the original graph structure \cite{xu21}.

\begin{figure}
\centering
\begin{tabular}{cc}
\includegraphics[width=1.45in]{5nodeGraph.pdf}&\includegraphics[width=1.7in]{5nodeGraph_plot.pdf}\\
\vspace{-0.25in}
\end{tabular}
\caption{\small Illustration of (a) a $5$-node line graph, (b) a $5$-node ring graph, where all nodes have the same degrees, and (c)  the first eigenvectors (\ie, 2D latent space vectors) of Laplacians of (a) and (b).}
\label{fig:4node_graph}
\vspace{-0.1in}
\end{figure}

\subsubsection{$2$-hop Neighbor Regularization}

However, objective \eqref{eq:obj1} is not sufficient---it does not consider \textit{second-order proximity} of the original graph $\cG$. 
Consider the simple $5$-node line graph example in Fig.\;\ref{fig:4node_graph}(a). 
Just requiring each connected node pair to be located in close proximity is not sufficient to uniquely result in a straight line solution (and thus in lowest dimensional latent space). 
For example, a zigzag line in 2D latent space is also possible.

Thus, we propose to regularize the objective \eqref{eq:obj1} using our second graph assumption: 
sparsity of the input manifold graph connectivity is determined based on point-to-point distance on the underlying manifold. 
This means that if $(i,j) \in \cE$ but $(i,l) \not\in \cE$, then distance $d_{i,j}$ between $(i,j)$ must be smaller than distance $d_{i,l}$ between $(i,l)$, or $d_{i,j} < d_{i,l}$. 

Based on this assumption, we define our regularizer $g(\P)$ as follows.
Denote by $\cT_i$ the \textit{two-hop neighbor} node set from node $i$ (\ie, node $j \in \cT_i$ is reachable in two hops from $i$, but $(i,j) \not\in \cE$).
The aggregate distance between each node $i$ and its 2-hop neighbors in $\cT_i$ is
\begin{align}
g(\P) = \sum_{i \in \cV} \sum_{j \in \cT_i} \|\p_i - \p_j \|^2_2 .
\label{eq:reg0}
\end{align}

We can write \eqref{eq:reg0} in matrix form.
For each $\cT_i$, we first define matrix $\bTheta_i \in \{0, 1\}^{N \times N}$ with entries

\vspace{-0.1in}
\begin{small}
\begin{align}
\Theta_{m,n} = \left\{ \begin{array}{ll}
1 & \mbox{if}~ m = n = i ~~~\mbox{or}~~~ m = n \in \cT_i \\
-1 & \mbox{if}~ m = i, n \in \cT_i ~~~\mbox{or}~~~ m \in \cT_i, n = i \\
0 & \mbox{o.w.}
\end{array} \right. .
\label{eq:Q}
\end{align}
\end{small}\noindent
We can then define $\Q = \sum_{i \in \cV} \bTheta_i$. 
The regularizer is thus $g(\P) = \text{tr}(\P^{\top} \Q \P)$, and the optimization becomes
\begin{align}
\min_{\P} &~ \text{tr}(\P^{\top} \L \P) - \mu \, \text{tr}(\P^{\top} \Q \P) 
= \text{tr} (\P^{\top} \underbrace{\left( \L - \mu \Q \right)}_{\A} \P )
\label{eq:obj2}
\end{align}
where $\mu > 0$ is a positive weight parameter to be discussed. 
Note that objective \eqref{eq:obj2} remains quadratic in variable $\P$. 

%The matrix version of the orthonormal requirement $\q_i^{\top} \q_j = \delta_{i-j}, \forall i,j$ is $\P \P^{\top} = \I$. The solution to the optimization is the first $K$ eigenvectors $\{\v_i\}_{i=1}^K$ of PSD matrix $\A = (\H - \bar{\W})^{\top} (\H - \bar{\W})$. Note that $\text{rank}(\A) = M$, and the dimension of null-space corresponding to eigenvalue $\lambda_1 = 0$ is $N-M$. 


\subsection{Choosing Weight Parameter $\mu$}

As a quadratic minimization problem \eqref{eq:obj2}, it is desirable for $\A = \L - \mu \Q + \epsilon \I$ to be \textit{positive semi-definite} (PSD) so that the objective is lower-bounded, \ie,  $\q^{\top} \A \q \geq 0, \forall \q \in \mathbb{R}^N$. 
We set $\epsilon = \lambda^{(2)}_{\min}(\Q)$ to be the \textit{second} smallest eigenvalue---the Fiedler number---of $\Q$ (Laplacian has $\lambda^{(1)}_{\min}(\Q) = 0$); larger $\lambda^{(2)}_{\min}(\Q)$ means more disconnected 2-hop neighbors, and a larger $\mu$ is desired. 
We compute $\mu > 0$ so that $\A$ is guaranteed to be PSD via GCT \cite{varga04}.
Specifically, we compute $\mu$ such that left-ends of all Gershgorin discs corresponding to rows of similarity transform $\S \A \S^{-1}$ of $\A$\footnote{Similarity transform $\S \A \S^{-1}$ and $\A$ have the same set of eigenvalues.}, where $\S = \text{diag}(\{s_i\})$ and $s_i > 0, \forall i$, are at least $0$. 
That means disc center $A_{i,i} \geq \sum_{j \neq i} |s_i A_{i,j} / s_j|$), or 
\begin{align}
L_{i,i} - \mu Q_{i,i} + \epsilon - \sum_{j | j \neq i} \left| \frac{s_i L_{i,j}}{s_j} - \mu \frac{s_i Q_{i,j}}{s_j} \right| & \geq 0, ~~\forall i .
\end{align}

Note that $L_{i,j} = -W_{i,j} \leq 0$, and $Q_{i,j} \leq 0$.
Note further that node $j$ cannot both be a $1$-hop neighbor to $i$ and a disconnected $2$-hop neighbor at the same time, and hence either $L_{i,j}=0$ or $Q_{i,j}=0$. 
Thus, we can remove the absolute value operator as
\begin{align}
L_{i,i} - \mu Q_{i,i} + \epsilon - \sum_{j | j \neq i} \left( -\frac{s_i L_{i,j}}{s_j} - \mu \frac{s_i Q_{i,j}}{s_j} \right) &\geq 0 .
\end{align}
We set the equation to equality and solve for $\mu_i$ for row $i$, \ie, 

\vspace{-0.15in}
\begin{small}
\begin{align}
\mu_i = \frac{L_{i,i} + \sum_{j|j\neq i} s_i L_{i,j}/s_j + \epsilon}{Q_{ii} - \sum_{j|j\neq i} s_i Q_{i,j} / s_j} 
%= \frac{\epsilon}{Q_{ii} - \sum_{j|j\neq i} Q_{i,j}} .
\label{eq:mu}
\end{align}
\end{small}\noindent
%where $L_{i,i} = - \sum_{j\neq i} L_{i,j}$.
Finally, we use the smallest non-negative $\mu = \min_{i} \mu_i$ for \eqref{eq:obj2}.


\subsection{Defining Orthogonality Condition}

%Computing latent coordinates $\p_i$'s using only objective \eqref{eq:obj2} and constraint $\P^{\top} \P = \I$ may be problematic. The reason is that constraint $\q_i^{\top} \q_j = \delta_{i-j}$ does imply the desirable condition $\q_i \neq \q_j$ for $i \neq j$, it is overly restrictive, resulting in \red{some examples?}. 

Instead of orthogonality condition $\q_i^{\top} \q_j = \delta_{i-j}$, we generalize the condition to $\q_i^{\top} \B \q_j = \delta_{i-j}$ for a chosen \textit{positive definite} (PD) matrix $\B$, which also implies the desirable $\q_i \neq \q_j$ for $i \neq j$.  
For simplicity, we choose $\B = \text{diag}(\{b_i\})$, where $b_i > 0, \forall i$, are scalars for the $N$ nodes. 
The constraint on variable $\P$ is now $\P \B \P^{\top} = \I$, which together with objective \eqref{eq:obj2} means computing the first $K$ \textit{generalized eigen-pair} for matrix pair $(\A, \B)$. 
We use LOBPCG \cite{lobpcg} for this task, running in $\cO(N)$ for sparse matrices, assuming $K \ll N$. 

For a given generalized eigen-pair $(\lambda_, \q)$ for matrix pair $(\A,\B)$ where $\B$ is PD and hence invertible, we can write
\begin{align}
\A \q &= \lambda \B \q \\
\B^{-1} \A \q &= \lambda \q .
\end{align}
Thus, $\q$ is also a \textit{right} eigenvector for asymmetric matrix $\B^{-1} \A$.
We determine scalars $\{b_i\}_{i=1}^N$ from this right eigenvector perspective.

We first observe that the numerator $\q^{\top} \A \q$ of the Rayleigh quotient for $(\A,\B)$ can be written as

\vspace{-0.05in}
\begin{small}
\begin{align}
\q^{\top} \A \q = \sum_{i \in \cV} \left( \sum_{j \in \cE_i} w_{i,j} (q_i - q_j)^2 - \mu \sum_{j \in \cT_i} (q_i - q_j)^2 \right)
\label{eq:contri}
\end{align}
\end{small}\noindent
where $\cE_i = \{j \,|\, (i,j) \in \cE\}$ is the set of $1$-hop neighbors of node $i$. 
The contribution for each node $i$ is indicated by the terms inside the bracket. 
In general, boundary nodes in the sampling domain have smaller degrees than interior nodes, as illustrated in Fig.\;\ref{fig:finite_graph}, and thus smaller contributions to the Rayleigh quotient.
As shown in the $5$-node line graph in Fig.\;\ref{fig:4node_graph}, because degrees of boundary nodes do not reflect the dimensionality of the underlying manifold, they create problems when deriving latent coordinates from computed eigenvectors; connected node-pairs in line graph are not evenly spaced (\eg, pair $(1,2)$ are closer than $(2,3)$), while the ring graph with no boundary nodes has no such problem.

We design scalars $\{b_i\}_{i=1}^N$ to remedy this problem. 
We first define \textit{generalized node degree} for node $i$ as the Gershgorin disc radius of row $i$ of $\B^{-1} \A$. 
We choose $\{b_i\}_{i=1}^N$ so that the generalized node degrees of all nodes are the same, while $\prod_{i=1}^N b_i = 1$.
Specifically, $r_1/b_1=r_2/b_2=\cdots=r_N/b_N$, where $r_i$ is the Gershgorin disc radius of row $i$ of $\A$. Then we have $b_1={r_1}/{(\prod_{i=1}^N{r_i})^{1/N}}$ and $b_i=r_ib_1/r_1$.

%\red{please fill in details}

==> response2reviewers_tsp/defs.tex <==
\def\0{{\mathbf 0}}
\def\1{{\mathbf 1}}

\def\a{{\mathbf a}}
\def\b{{\mathbf b}}
\def\c{{\mathbf c}}
\def\d{{\mathbf d}}
\def\e{{\mathbf e}}
\def\f{{\mathbf f}}
\def\g{{\mathbf g}}
\def\h{{\mathbf h}}
\def\i{{\mathbf i}}
\def\j{{\mathbf j}}
\def\k{{\mathbf k}}
\def\l{{\mathbf l}}
\def\m{{\mathbf m}}
\def\n{{\mathbf n}}
\def\o{{\mathbf o}}
\def\p{{\mathbf p}}
\def\q{{\mathbf q}}
\def\r{{\mathbf r}}
\def\s{{\mathbf s}}
\def\t{{\mathbf t}}
\def\u{{\mathbf u}}
\def\v{{\mathbf v}}
\def\w{{\mathbf w}}
\def\x{{\mathbf x}}
\def\y{{\mathbf y}}
\def\z{{\mathbf z}}

\def\A{{\mathbf A}}
\def\B{{\mathbf B}}
\def\C{{\mathbf C}}
\def\D{{\mathbf D}}
\def\E{{\mathbf E}}
\def\F{{\mathbf F}}
\def\G{{\mathbf G}}
\def\F{{\mathbf F}}
\def\H{{\mathbf H}}
\def\I{{\mathbf I}}
\def\J{{\mathbf J}}
\def\K{{\mathbf K}}
\def\L{{\mathbf L}}
\def\M{{\mathbf M}}
\def\N{{\mathbf N}}
\def\O{{\mathbf O}}
\def\P{{\mathbf P}}
\def\Q{{\mathbf Q}}
\def\R{{\mathbf R}}
\def\S{{\mathbf S}}
\def\T{{\mathbf T}}
\def\U{{\mathbf U}}
\def\V{{\mathbf V}}
\def\W{{\mathbf W}}
\def\X{{\mathbf X}}
\def\Y{{\mathbf Y}}
\def\Z{{\mathbf Z}}


\def\rE{{\text{E}}}
\def\rPr{{\text{Pr}}}
\def\Tr{{\text{Tr}}}
\def\vec{{\textrm{vec}}}
\def\ie{{\textit{i.e.}}}
\def\eg{{\textit{e.g.}}}


\def\cA{{\mathcal A}}
\def\cB{{\mathcal B}}
\def\cC{{\mathcal C}}
\def\cD{{\mathcal D}}
\def\cE{{\mathcal E}}
\def\cF{{\mathcal F}}
\def\cG{{\mathcal G}}
\def\cH{{\mathcal H}}
\def\cI{{\mathcal I}}
\def\cK{{\mathcal K}}
\def\cL{{\mathcal L}}
\def\cM{{\mathcal M}}
\def\cN{{\mathcal N}}
\def\cO{{\mathcal O}}
\def\cP{{\mathcal P}}
\def\cQ{{\mathcal Q}}
\def\cR{{\mathcal R}}
\def\cS{{\mathcal S}}
\def\cT{{\mathcal T}}
\def\cU{{\mathcal U}}
\def\cV{{\mathcal V}}
\def\cW{{\mathcal W}}
\def\cX{{\mathcal X}}
\def\cY{{\mathcal Y}}
\def\cZ{{\mathcal Z}}


\def\bpi{{\pmb{\pi}}}
\def\bphi{{\pmb{\phi}}}
\def\bpsi{{\pmb{\psi}}}
\def\bphi{{\pmb{\phi}}}
\def\bpsi{{\pmb{\psi}}}
\def\balpha{{\boldsymbol \alpha}}
\def\bbeta{{\boldsymbol \beta}}
\def\bmu{{\boldsymbol \mu}}
\def\btheta{{\boldsymbol \theta}}
\def\bupsilon{{\pmb{\upsilon}}}
\def\bvarphi{{\boldsymbol \varphi}}
\def\bLambda{{\boldsymbol \Lambda}}
\def\bPhi{{\boldsymbol \Phi}}
\def\bOmega{{\boldsymbol \Omega}}
\def\bPsi{{\boldsymbol \Psi}}
\def\bSigma{{\boldsymbol \Sigma}}
\def\bTheta{{\boldsymbol \Theta}}


\def\bcdot{{\;\boldsymbol{\cdot}\;}}

==> response2reviewers_tsp/reviewer_1.tex <==
{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 1:}
The authors focus on manifold graphs to gradient graph Laplacian regularizer that provably promotes piecewise planar signal reconstruction.

1. Technical contributions are supposed to be further refined.
}\vspace{\comafter}

\noindent\textbf{Response 1:}
In the revised manuscript, we have refined the list of our contributions at the end of the Introduction. 
\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 2:}
2. Better to switch the sections ``II. RELATED WORKS'' and ``III. PRELIMINARIES'', particularly to introduce scientific motivation on how to deal with the well-known ``staircase'' effect.
}\vspace{\comafter}

\noindent\textbf{Response 2:}
We thank the reviewer for the suggestion. 
However, we feel that keeping the discussion on related works in Section\;II would immediately provide proper context to understand our key contributions listed in the Introduction.
As for the well-known ``stairecase" effect, we have modified the Introduction to state that it is illustrated in forthcoming Fig.\;6 and 10 to facilitate understanding in the revised manuscript. 
\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 3:}
3. The innovation itself might not be as apparent as the authors described.
}\vspace{\comafter}

\noindent\textbf{Response 3:}
In the revised manuscript, we have restated our contributions more clearly at the end of the Introduction. 
\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 4:}
Overall, the presented study is possible to be further improved in a fascinating story, so expect future versions of this manuscript.
}\vspace{\comafter}

\noindent\textbf{Response 4:}
We thank the reviewer for the positive comments. 
we have made significant improvement to address all reviewers' comments in the revised manuscript to improve the overall story.
\vspace{\resafter}

==> response2reviewers_tsp/reviewer_2.tex <==
{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 1:}
The paper concerns application of the gradient graph Laplacian regularization technique to manifold graph signal restoration. The text is quite well written and technically sound. I would however, consider shortening the text due to its limited contribution and publishing it as a letter.  
}\vspace{\comafter}

\noindent\textbf{Response 1:}
We thank the reviewer for the positive comment on the readability of our paper.
However, with due respect to the reviewer, given the limited and sometimes technically incorrect comments provided below, we are concerned whether the reviewer understood our paper sufficiently to qualify our contributions ``limited". 

\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 2:}
All the claims that are named Theorems in this article are trivial properties of the matrices at hand. For example, Theorem 1 plainly states that given a PSD matrix L, its conjugation by F yields a PSD matrix. This property of PSD matrices in demonstrated in every undergraduate Linear Algebra course through a simple change of basis. How can the authors claim it as their theorem? Same for Theorem 2 and all other Theorems - these are trivial properties and must be marked as such. 
}\vspace{\comafter}

\noindent\textbf{Response 2:}

With due respect to the reviewer, in our humble opinion this blanket statement that ``all the claims that are named Theorems are trivial properties of the matrices at hand" is an unjustified and gross over-simplification of our contributions in the paper with scant evidence provided, while overlooking a large fraction of the manuscript (roughly 40\%) that was never mentioned. 
For example, a key concept of the paper is \textit{graph embedding} (the entire Section VI)---computation of latent coordinates of a manifold graph given only an undirected graph with connectivity and positive edge weights. 
This was never mentioned by the reviewer. 
Consider also the derivation of the optimal tradeoff parameter $\mu$ that optimally trades off the fidelity term and the proposed GGLR regularization (the entire Section V, including Theorem 4) through a careful analysis of the bias-variance tradeoff. 
This was also never mentioned by the reviewer.
The reviewer provided no evidence that Theorem 4 in Section V constitutes ``trivial properties of the matrices at hand".  
The reviewer also provided no evidence that Theorem 3 in Section IV-G, which requires an elaborate half-page proof in Appendix B, constitutes ``trivial properties of the matrices at hand".  
Further, the reviewer provided no evidence that Theorem 2 in Section IV constitutes ``trivial properties", which requires Lemma 3 in the same section that itself is non-trivial.

Reviewer focused his/her argument on the proof of Theorem 1 (since expanded in the revised manuscript to include a related claim that GGLR promotes planar signal reconstruction). 
While the proof for the first half is indeed straightforward, we wrote only two lines of mathematical derivation and included it here for completeness. 
Just by removing two lines of a 16-page manuscript would not reduce the volume of the paper to a letter.
Moreover, we call this result a ``Theorem" not for the complexity of its proof, but for its practical importance: as a regularizer of the form $\x^\top \cL \x$ for a minimization objective, it is critical that $\cL$ is PSD so that $\x^\top \cL \x \geq 0, \forall \x$.
Its importance is evident in the following section when a MAP objective is formulated using GGLR for regularization.
(Further, Theorem 1 is used in the proof of Theorem 3 in Appendix B). 
Finally, Theorem 1 enables a new construction of a \textit{signed} graph with a Laplacian matrix that is provably PSD, which differs from previous studies of Laplacians of signed graphs in the GSP literature.
We humbly ask the reviewer to read carefully the Remarks immediately following Theorem 1 for details to appreciate its importance in this GSP context.
\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 3:}
Further, Lemma 2 is a known Ordinary Least Squared with Ridge regularization result. No proof is needed while reference to the source is mandatory. 
}\vspace{\comafter}

\noindent\textbf{Response 3:}
With due respect to the reviewer, the reviewer is technically incorrect here. \textit{Ridge regression}\footnote{https://en.wikipedia.org/wiki/Ridge\_regression} refers to the addition of a scalar times an identity matrix, $k*\I$, to the coefficient matrix of an ordinary least square (OLS) estimator to improve conditioning:
\begin{align}
\hat{\bbeta} = (\X^\top \X + k \I)^{-1} \X^\top \y .
\end{align}
The name ``ridge" refers to the shape of the diagonal of $\I$. 
In this case, $\X^\top \X$ is clearly PSD, and adding a PD $k \I$ will clearly result in a PD matrix, making it invertible. 
Here, indeed no proof is necessary. 
In contrast, however, \textit{equation (31) in Theorem 3 in the revised manuscript is clearly NOT an OLS estimator with an added scaled identity matrix}. 
Specifically, while GNG Laplacian $\cL$ is PSD (as stated in much maligned Theorem 1), $\H^\top \H$ is clearly NOT a scaled identity and NOT full-rank in the general case (note the difference between ``full rank" and ``full row-rank" for a rectangular fat matrix). 
We humbly ask the reviewer to read the elaborate half-page proof in Appendix B carefully. 

\vspace{\resafter}

{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 4:}
Same applied tot he rest of the text - kindly cite the sources and avoid proofs of well known claims. This will significantly reduce the volume.
}\vspace{\comafter}

\noindent\textbf{Response 4:}
With due respect to the reviewer, we humbly ask the reviewer to carefully read the \textit{entire} text of our submitted paper and offer professional comments on all sections (rather than cherry-picking one isolated two-line proof and extrapolating based on evidence-free conjectures), including the significantly revised Section 4 (GGLR for Graphs with Coordinates), Section 5 (Computation of Optimal Tradeoff Parameter) and Section 6 (Computation of Latent Coordinates), the later two section took up roughly $40\%$ of the technical content but received no comments from the reviewer in the first review round. 
\vspace{\resafter}


==> response2reviewers_tsp/reviewer_3.tex <==
{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 1:}
The authors present a Gradient graph laplacian regulariser for recovery of signals over graphs.
The manuscript reads well and is mostly easy to follow. 
}\vspace{\comafter}

\noindent\textbf{Response 1:}
We thank the reviewer for the positive comment on the readability of our manuscript. 


\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 2:}
However, I have questions regarding the following main aspects.
The entire work hinges on the concept of planar graph signals — However, it is never clearly defined though it is mentioned all over the place. The first mention of discussion of PWP appears on page 5: 'we discuss PWP in Section IV-E. ‘But in that Section, we find it already being used conceptually, and not defined as a concept. Indeed, it became a bit evident only from the paragraph below Figure 4: ‘In Fig. 4(e), we see that neighboring nodes have the same gradients except node (2,3). ‘— that perhaps the idea is to enforce smoothness of the gradient of the signal? 
}\vspace{\comafter}

\noindent\textbf{Response 2:}
We apologize for not providing a clear definition of a planar graph signal from the beginning in the original manuscript, which would have indeed clarified many of the reviewer's misunderstandings (see our responses below). 
In the revised manuscript, we have added clear definitions of planar / piecewise planar signals with respect to (w.r.t.) a set of latent coordinates in Section III-B. 
The notion of \textit{manifold gradient} defined w.r.t. global coordinates is a key concept in the paper and very different from conventional \textit{graph gradients} computed using conventional adjacency or graph Laplacian matrix (see our response 3 below for a detailed exposition). 
This notion of manifold gradient is motivated by practical applications in 2D images and 3D point clouds that can reasonably be interpreted as discrete samples on continuous manifolds, both of which have employed graphs as an abstraction for processing in recent years \cite{osher2017low,zeng20193d,hu2021dynamic}. 
We demonstrate the usefulness of our manifold gradient notion in the experimental section.
\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 3:}
This further prompts to this simpler view of the problem, would a regularisation such as $(\x-\A\x)^\top \L (\x-\A\x)$ not have the same effect, given that the goal is to enforce smoothness on the residual or edge or gradient, $(\x-\A\x)$ approximating the backward difference gradient over the graph? 
}\vspace{\comafter}

\noindent\textbf{Response 3:}
We thank the reviewer for the suggestion, which shows that we did not successfully convey the importance of our \textit{manifold gradient} notion in our original manuscript, for which we apologize. 
We can demonstrate the fallacy of the reviewer's suggestion through a very simple example. 
Consider a 3-node line graph with edges connecting nodes $(1,2)$ and $(2,3)$ with weight $1$, and an accompanied graph signal $\x = [2, 0, -2]^\top$. 
Plotting signal value versus signal index, we clearly see a linear line. 
In this case, the adjacency, degree, and graph Laplacian matrices are
\begin{align}
\A = \left[ \begin{array}{ccc}
0 & 1 & 0 \\
1 & 0 & 1 \\
0 & 1 & 0
\end{array} \right], ~~ 
\D = \left[ \begin{array}{ccc}
1 & 0 & 0 \\
0 & 2 & 0 \\
0 & 0 & 1
\end{array} \right], ~~
\L = \left[ \begin{array}{ccc}
1 & -1 & 0 \\
-1 & 2 & -1 \\
0 & -1 & 1
\end{array} \right].
\end{align}
However, computing $\A \x = [0, 0, 0]^\top$ and $\x - \A \x = [2, 0, -2]^\top$, we clearly see that $(\x - \A\x)^\top \L (\x - \A\x) = 8 > 0$. This would be true even if a normalized version of the adjacency matrix is used, for example, row-stochastic $\A_r = \D^{-1} \A$.

In contrast, given a set of 1-dimensional latent coordinates $(1), (2), (3)$ for the three nodes respectively, we use our proposed procedure to construct a DAG $\cG^d$, define a gradient computation operator $\G$, a gradient graph $\bar{\cG}$ of two nodes with Laplacian $\bar{\L}$, and finally a GNG Laplacian $\cL$, 
\begin{align}
\G = \left[ \begin{array}{ccc}
1 & -1 & 0 \\
0 & 1 & -1
\end{array} \right], ~~~
\bar{\L} = \left[ \begin{array}{cc}
1 & -1 \\
-1 & 1
\end{array} \right], ~~~
\cL = \left[ \begin{array}{ccc}
1 & -2 & 1 \\
-2 & 4 & -2 \\
1 & -2 & 1
\end{array} \right] .
\end{align}
Using GLG Laplacian $\cL$, we can compute a GGLR value $\x^\top \cL \x = 0$, which agrees with our intuition for a linear line. 
The reason we can compute a more reasonable regularizer for a linear line is because we computed manifold gradients w.r.t. latent coordinates that are defined globally. 
In contrast, the graph gradients computed using the reviewer's proposed $\x - \A \x$ are computed w.r.t. individual nodes with no global directionality. 
This example clearly demonstrates the fallacy of the reviewer's suggestion.

In the revised manuscript, we have added a new Section IV-A titled ``Why Graph Laplacian cannot promote Planar Signals" to explain the difficulty of defining a planar / linear signal using exclusively the Laplacian operator.
We humbly ask the reviewer to read that section for details.

\vspace{\resafter}



{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 4:}
Coming back to the application on 2D and 3D images, I was also reminded of approaches that create smoothened edge-maps, some of which are also cited to in the paper. How is the conceptual novelty of the proposed work over them — in precise terms, what is the motivation for the specific gradient graph and the PWP concepts is never made clear. 
}\vspace{\comafter}

\noindent\textbf{Response 4:}
We are unsure what the reviewer meant by ``smoothened edge-maps" with no mention of specific papers. 
Searching among our cited references, we conjecture that the reviewer is referring to \textit{bilateral filter} (BL) \cite{tomasi98} that preserves edges while denoising an image. 
It has been shown that BL promotes PWC signal reconstruction \cite{pang17,liu17}, and thus its effectiveness is related to SDGLR. 
It is also well known that BL suffers from the ``staircase" effect as discussed in the Introduction and shown in Fig.\;6(f) and Fig.\;10. 
As discussed in the Introduction and shown in new Fig.\;1, many graph signals are slowly varying across the underlying kernels, and promoting PWC signal reconstruction is clearly not suitable. 
This motivates a generalization to promote PWP signal reconstruction instead.
This discussion is included in the new Introduction of the revised manuscript.
\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 5:}
For example, why are PWP signals important in real-world settings? 
}\vspace{\comafter}

\noindent\textbf{Response 5:}
There exist many practical graph signals that are slowly varying across the underlying kernels with occasional discontinuities; see the new Fig.\;1 in the revised manuscript for examples.
PWP signals---generalizing from PWC signals---have been shown to be useful models for 2D imaging for over a decade; see for example works on \textit{total generalized variation} (TGV) \cite{bredies2010total, bredies2015tgv} that generalizes \textit{total variation} (TV) \cite{chambolle1997image,selesnick2014convex} (which promotes PWC signal reconstruction) and similarly promotes PWP signals in 2D images.  
Note that we have already juxtaposed our proposed SDGGLR with TGV in the related work section.
We repeat our discussion here for the reviewer's perusal.

\vspace{0.1in}
\begin{quote}
Its generalization, \textit{total generalized variation} (TGV) [16], [17], better handles the known staircase effect, but retains the non-differentiable $\ell_1$-norm that requires iterative optimization. 
Like TGV, GGLR also promotes PWP
signal reconstruction, but is non-convex and differentiable.
This leads to fast optimizations to be discussed later.
\end{quote}
\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 6:}
How does the spectrum of the gradient graph Laplacian relate to that of the underlying actual graph Laplacian’s spectrum? 
}\vspace{\comafter}

\noindent\textbf{Response 6:}
We thank the reviewer for this comment. 
We have already provided partial answer to question in Section IV-E of the revised manuscript. 
\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 7:}
Can we infer some intuition on when are where the two graphs can provide complementary information? As in, where would it be necessary to use the SDGGLR and not the SDGLR (From the numerical experiments it seems that mostly their performance is similar in both PSNR and SSIM). 
}\vspace{\comafter}

\noindent\textbf{Response 7:}
First, we respectfully disagree with the reviewer's comment that the performance of SDGGLR and SGLR are similar.
In the revised Table III, we see that for image interpolation, the performance of SDGGLR exceeded that of SGLR for \textit{all} images at \textit{all} missing pixel percentages, by up to $2.45$dB in PSNR. 
In the revised Table V, for point cloud denoising the performance gain is up to $2.09$dB in PSNR.
These are not trivial gains in imaging; for example, the PSNR gain from video compression standard H.264 to HEVC at the same bitrates, after more than a decade of video coding development, is roughly $2$dB.
The differences in PSNR in Table VI and VIII for graph signals without latent coordinates are even more significant (by near 4dB on average).
Finally, the visual differences between SDGGLR and SDGLR in Fig.\;10 for image patch denoising and interpolation are stunningly obvious.

A signal that is PWC is also non-continuous PWP (see new Section IV-F for a detailed discussion on piecewise planar signal reconstruction). 
Thus, if latent coordinates can be reasonably obtained, one would employ SDGGLR over SDGLR.
For graphs that do not naturally have latent coordinates as attributes, and they are not manifold graphs, then reasonable latent coordinates cannot be easily obtained using our proposed method in Section VI. 
In such cases, obviously one would choose SDGLR over SDGGLR.
\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 8:}
Side note: What is SSIM? (Not defined). 
}\vspace{\comafter}

\noindent\textbf{Response 8:}
Structural similarity index measure (SSIM) \cite{wang2004image} is an exceedingly common objective image quality assessment metric in the image processing literature. 
Besides Peak Signal-to-Noise Ratio (PSNR), SSIM is by far the most prevalent image quality measure that is used in the imaging community today. 
We have provided appropriate reference in the revised manuscript. 
\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 9:}
So when does the user prefer SDGGLR over SDGLR? Such considerations would really help the reader see the merits and understand the intuition behind the concepts.
}\vspace{\comafter}

\noindent\textbf{Response 9:}
See our response to comment 7 above.
\vspace{\resafter}



\vspace{0.5in}

{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 1:}
What is the staircase effect? Please explain or illustrate — referred to everywhere but never told what it is.
}\vspace{\comafter}

\noindent\textbf{Detailed Response 1:}
In the original manuscript, the ``staircase" effect was illustrated in Fig.\;4(f) with a forward point in footnote 2 in the Introduction.
In the revised manuscript, it is illustrated in Fig.\;6(f) and and Fig.\;10.
%In fact, in footnote 2, it was written ``This will be illustrated in details later in Fig. 4.". 


\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 2:}
What is piecewise planar signal definition?
What is the motivation of considering PWP? 
}\vspace{\comafter}

\noindent\textbf{Detailed Response 2:}
Definitions of planar and piecewise planar (PWP) signals are provided in Section III-B of the revised manuscript.
There exist many practical graph signals that are slowly varying across the underlying kernels with occasional discontinuities; see the new Fig.\;1 in the revised manuscript for examples.
PWP signals---generalizing from PWC signals---have been shown to be useful models for 2D imaging for over a decade; see for example works on \textit{total generalized variation} (TGV) \cite{bredies2010total, bredies2015tgv} that generalizes \textit{total variation} (TV) \cite{chambolle1997image,selesnick2014convex} (which promotes PWC signal reconstruction) and similarly promotes PWP signals in 2D images.  

\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 3:}
The section on Gerschgorin Circle theorem seems irrelevant and hanging. The ideas are used later in experiments but never explained clearly.
}\vspace{\comafter}

\noindent\textbf{Detailed Response 3:}
Gershgorin circle theorem (GCT) (summarized in Section III-C) is relevant and is used in Section VI-C to compute parameters for our proposed graph embedding algorithm. 
We added a forward pointer in Section III-C to alert readers when GCT will be used in the sequel. 

\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 4:}
I feel that the example in figure 1, though simple, is not sufficient to demonstrate the concepts.
}\vspace{\comafter}

\noindent\textbf{Detailed Response 4:}
Fig.\;2 in the revised manuscript (Fig.\;1 in the original paper) is used to illustrate the effectiveness of SDGLR in promoting PWC signal reconstruction.
Specifically, in Fig.\;2(c), it is visually very clear that the noisy signal (black) was restored to a PWC signal (red).  
We believe that a fair-minded reader would understand the simple illustration of PWC signal reconstruction.
We are confused as to why the reviewer feels this is not sufficient, and the reviewer provided no further explanation.

\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 5:}
On page 4: Sec A— is finding a DAG for a given graph a computationally feasible problem always? Specially not just one DAG, but $k$ DAGS? Are the DAGS always guaranteed to be connected — or is it necessary for the analysis that follows?
}\vspace{\comafter}

\noindent\textbf{Detailed Response 5:}
Given an undirected graph $\cG(\cV,\cE,\W)$ and associated latent coordinates $\{\p_i\}$ for all nodes $i \in \cV$, the redesigned DAG construction procedure described in Section IV-B of the revised manuscript is employed so each node $i$ can identify $K^+ \geq K$ neighbors to properly compute manifold gradient $\balpha^i \in \mathbb{R}^K$ via equation (16).
Given $\cO(N)$ nodes can identify $K^+$ neighbors satisfying the \textit{acyclic condition} stated in the procedure, the complexity of the DAG construction is $\cO(NK^+)$.
In response to the reviewer's comment, in the revised Section\;IV we construct only one DAG $\cG^d$, and thus one gradient graph $\bar{\cG}$, and one GNG Laplacian $\cL$ for GGLR regularization, reducing the complexity of overall graph construction. 
 
DAG $\cG^d$ is only used to identify $K^+$ neighbors for each node $i$ to compute manifold gradient $\balpha^i$; whether $\cG^d$ is overall connected or not is irrelevant. 

\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 6:}
I also did not get why the DAGs have been introduced — what is the interpretation/intuition behind the ‘directionality’ that the authors claims it imposes, specially when the underlying graph is undirected?
}\vspace{\comafter}

\noindent\textbf{Detailed Response 6:}
We first refer the reviewer back to our earlier response to detailed comment 5, where the purpose of the DAG is explained. 
Like the 4-node line graph in Fig.\;4(a) that has only 3 unique slopes, the acyclic nature of the constructed DAG (as stated in the new Lemma 1 of the revised manuscript) ensures that each computed manifold gradient $\balpha^i$ is unique and not duplicated.
\vspace{\resafter}



{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 7:}
‘If there are more than one sink in … to create a unique sink at $\I^*$’— unclear.
What is the role of this sink?
}\vspace{\comafter}

\noindent\textbf{Detailed Response 7:}
To simplify technical presentation, we have removed the notion of a sink node in the revised manuscript. 

\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 8:}
What is exactly the motivation behind the operator $\F$ in eq(8) — what is it capturing? How is it related to $\L$, given that the regular graph-Laplacian is itself interpretable as a gradient operation, what is the added information obtained from $\F$?
}\vspace{\comafter}

\noindent\textbf{Detailed Response 8:}
We first refer the reviewer to Section IV-A titled ``Why Graph Laplacian cannot promote Planar Signals", containing a detailed examination of the fallacy of using graph Laplacian to compute graph gradients for promotion of PWP signals. 
Given the shortcomings of $\L$, the purpose of a gradient operator $\F^i$ for node $i$, defined in equation (12) of the revised manuscript, is to compute a manifold gradient $\balpha^i \in \mathbb{R}^K$ at node $i$ via equation (16) that are least-square minimizing parameters of a best-fitted hyperplane model in equation (6).

\vspace{\resafter}



{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 9:}
Lemma 1: What is the Lemma telling us?
}\vspace{\comafter}

\noindent\textbf{Detailed Response 9:}
The interpretation of Lemma 3 of the revised manuscript (Lemma 1 of the original paper) is elaborated in the ``Remarks" following the proof. 
We repeat the content here for the reviewer's perusal. 

\vspace{0.1in}
\begin{quote}
(23) states that the constant signal $\1$ has zero gradient. 
Further, (23) implies that $\G(\x + c \1) = \G \x, \forall \x \in \mathbb{R}^N, c \in \mathbb{R}$, \ie, gradient computation $\G$ is invariant to constant shift on signal $\x$.
(23) also means that any constant vector is in the \textit{nullspace} of $\G$. 
\end{quote}
Note that ``Remarks" are consistently provided after the lemmas and theorems precisely to provide intuitive interpretations. 

\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 10:}
‘Because $\G^k$ is a DAG, nodes can be renumbered’… isn’t the numbering subject to being same across different $k$?
}\vspace{\comafter}

\noindent\textbf{Detailed Response 10:}
We assume the reviewer is referring to the proof of Lemma 3 of the revised manuscript. 
The reviewer has misunderstood.
The purpose of the node renumbering inside the proof is to prove the second property in equation (24): $\text{rank}(\G) = N-1$. 
Node renumbering translates to reordering rows/columns of matrix $\G$, which does not affect the rank of $\G$. 
Thus, proving a reordered $\G$ has rank $N-1$ implies the original $\G$ is also rank $N-1$. 
No node renumbering or rows/columns reordering is actually performed in practice. 
\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 11:}
Page 6: Sec B: ‘To promote planar signal reconstruction ‘— why do you promote it? What is it conceptually?
}\vspace{\comafter}

\noindent\textbf{Detailed Response 11:}
When adding a non-negative signal prior term $\text{Pr}(\x)$, $\text{Pr}(\x) \geq 0, \forall \x$, to a minimization objective $f(\x)$, resulting in optimization of the form
\begin{align}
\min_{\x} f(\x) + \mu \, \text{Pr}(\x),    
\label{eq:opt}
\end{align}
where $\mu > 0$ is a tradeoff parameter, 
the goal is to introduce a \textit{bias} in the solution space, so that one would prefer solution $\x_1$ over $\x_2$ if $f(\x_1) = f(\x_2)$ and $\text{Pr}(\x_1) < \text{Pr}(\x_2)$.
In other words, the optimization \eqref{eq:opt} is biased towards solutions $\x$ with small $\text{Pr}(\x)$ over solutions with large $\text{Pr}(\x)$, or more simply, the optimization \textit{promotes} solutions $\x$ with small $\text{Pr}(\x)$.
We have added an explanation of the term ``promote" as a footnote in the Introduction: 

\vspace{0.05in}
\begin{quote}
By ``promote” we mean adding a non-negative signal prior $\text{Pr}(\x)$ to a minimization objective $f(\x)$ to bias the solution $\x$ towards small $\text{Pr}(\x)$.    
\end{quote}
Note that the terminology ``promote" is consistent with the GSP literature when discussing regularizers, for example, \cite{yankelevsky16}, \cite{mahmood18}, \cite{liu19depth}, Pg.41, Pg.50, Pg.146, Pg.147, Pg.148, Pg.149, Pg.150, Pg.152, Pg.204 in \cite{cheung21}.
Thus, we believe that our usage of the term ``promote" is well justified and consistent with the existing literature.

In practice, one would introduce such term if there is \textit{a priori} knowledge about the sought solution $\x$. 
In this paper, we assume that the solution $\x$ follows a planar / piecewise planar (PWP) model as described in Section III-B of the revised manuscript, generalizing from previous piecewise constant (PWC) model. 
For 2D images, PWP is a common assumption and was promoted mathematically using \textit{total generalized variation} (TGV) previously \cite{bredies2010total, bredies2015tgv}. 
See the new Fig.\;1 for practical examples of slowly varying signals over graph kernels with occasional discontinuities fitting this PWP model. 
Our proposal of GGLR is suitable for restoration of signals fitting this PWP model, as demonstrated in four applications in the results section. 

\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 12:}
In Theorem 1: By definition: $\cL^k=..$, is it by construction? The equation was not immediate to me.
}\vspace{\comafter}

\noindent\textbf{Detailed Response 12:}
In the revised manuscript, the definition of GNG Laplacian $\cL = \G^\top \R^\top \bar{\L}^o \R \G$ is stated in equation (22) just above Theorem 1.
\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 13:}
‘In contrast, a GNG—as shown in Fig. 2(d)—has no self-loops and is not balanced in general, yet its corresponding GNG Laplacian is provably PSD.
‘ — what is the impact of the balanced-ness on the analysis? On the spectral properties?
}\vspace{\comafter}

\noindent\textbf{Detailed Response 13:}
The statement contrasts the current work with a previous work \cite{yang21} that studies balanced signed graphs. 
Laplacian matrices for signed graphs can be negative definite (while Laplacians of positive graphs are always PSD \cite{cheung18}). 
However, we show in Theorem 1 that that our GNG Laplacian matrix is provably PSD, and we do not rely on the graph balance analysis in \cite{yang21} to do so.
More generally, we refer the reviewer to revised ``Remarks" below Theorem 1 for an exposition of the proposed GNG Laplacian in relations to Laplacians of signed graphs studied in the GSP literature.   
\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 14:}
The authors should try to tell us if the GNG Laplacians $\cL^k$ (Theorem 2) have any explicit connections to the true graph Laplacian $\L$, e.g., the spectrum, the eigenvectors, eigenvalues, — or in terms on hops, neighbourhoods …

What is the Theorem 2 intuitively telling us?
}\vspace{\comafter}

\noindent\textbf{Detailed Response 14:}
We are unsure what the reviewer is asking for.
Why must the graph Laplacian $\L$ for the original graph $\cG$ have ``explicit connections" with the GNG Laplacian for the gradient induced graph (GNG) $\cG^*$ either in the spectral domain or the nodal domain? 
For regularization, the two Laplacians serve two different purposes: GLR $\x^\top \L \x$ promotes PWC signal reconstruction, and GGLR $\x^\top \cL \x$ promotes PWP signal reconstruction via PWC manifold gradient reconstruction.

As done consistently following lemmas sand theorems in the paper, the intuition provided by Theorem\;2 is already elaborated in the following ``Remark" paragraph, which we repeat here for the reviewer's perusal. 

\begin{quote}
Given Theorem\;2, one can see that multiplying $\cL$ by any linear combination $\v = \alpha_1 \v_1 + \alpha_2 \v_2$ of the first two eigenvectors $\v_1$ and $\v_2$ (corresponding to eigenvalue $0$) will also result in $\0$. 
Using our 4-node line graph in Fig.\;4(a) as example, $\v_2 = [1.5 ~0.5 ~-0.5 ~-1.5]^{\top}$. 
We see that any linear combination of $\v_1$ and $\v_2$ is a straight line.
This agrees with our intuition that 1D GGLR promoting linear signal reconstruction should evaluate to $0$ for any linear signal. 
\end{quote}

\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 15:}
The condition of rank 2 in Lemma2, (a) is it that reasonable to be ‘typically satisfied’ as claimed by authors? (b) what does it imply in terms of the signal properties?
}\vspace{\comafter}

\noindent\textbf{Detailed Response 15:}
For clarification, we have rewritten the ``Remarks" paragraph following Theorem 3 in the revised manuscript (Lemma 2 in the original paper) as follows:

\begin{quote}
(31) can be solved as a linear system $\bPhi \x^* = \H^\top \y$ efficiently without matrix inverse using CG \cite{axelsson1986rate}.  
The first condition means that $M$ rows of $\H$ ($M$ observations) are linearly independent. 
The condition $\H \v_i \neq \0$ means that eigenvectors $\{\v_i\}$ of $\cL$ for eigenvalue $0$ cannot be unobservable. 
The second condition means that the projections of orthogonal eigenvectors $\{\v_i\}$ onto the row space $\cR(\H)$ of $\H$ must remain mutually linearly independent.
For denoising $\H = \I$, and the conditions are trivially true.
For interpolation $\H^\# \H$ is a diagonal matrix of ones and zeros, and the conditions are true for large enough $M$.
For deblurring $\H$ is often a low-pass filter, and the second condition is typically true given $\{\v_i\}$ are smooth vectors combined to describe a planar signal.
\end{quote}
\vspace{\resafter}



{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 16:}
‘Condition requiring….linearly independent’ — unclear
}\vspace{\comafter}

\noindent\textbf{Response 16:}
See our response to detailed comment 15 above.

\vspace{\resafter}



{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 17:}
What is the performance when $\mu$ =0 for the House example. Also, what is the House image? Please show.
}\vspace{\comafter}

\noindent\textbf{Detailed Response 17:}
Setting $\mu = 0$ would mean no signal prior is applied, and thus the optimization in equation (30) becomes ill-posed and not solvable. 
Thus, no solution image can be generated to compute a MSE as performance.
We have added the \texttt{House} image in the revised manuscript. 
\vspace{\resafter}



{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 18:}
It seems odd that you first solve for the $\x^*$ using (25) assuming constant $\mu$ and then later minimise the MSE— its a suboptimal step — why not solve the entire problem using gradient descent on all the relevant parameters together? (As hinted by the authors in the last sentence before Section VI)?
}\vspace{\comafter}

\noindent\textbf{Detailed Response 18:}
There is a misunderstanding here; we do not solve for $\x^*$ using (32) at all.
We first compute an ``optimal" tradeoff parameter $\mu$ by minimizing $MSE^a(\mu)$ via \textit{accelerated gradient descent} (AGD), then the computed $\mu$ is used to properly pose the optimization in (30), where the solution is in (31).

\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 19:}
Fig 5: Please consider enlarging the fonts — nothing is readable in print.
}\vspace{\comafter}

\noindent\textbf{Detailed Response 19:}
We have increased the font sizes for Fig.\;7 in the revised manuscript (Fig.\;5 in the original manuscript).
\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 20:}
In page 8: ‘inputted’ is not a valid usage — used as input is better.
}\vspace{\comafter}

\noindent\textbf{Detailed Response 20:}
We do not understand why ``inputted" is not a valid usage here. 
According to the Marriam-Webster dictionary\footnote{https://www.merriam-webster.com/dictionary/input}, ``input" can be used as a transitive verb, as shown in the provided example in the webpage: ``She inputted the sales figures into the spreadsheet."
In our case, we are using ``inputted" in passive voice.
\vspace{\resafter}




{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 21:}
Perhaps the authors can tell us what it is about the discarded graphs in Table II that makes them a bad candidate more intuitively. More generally, does the VBC translate to some constraints on structure of the ‘good graphs’ — for example, will it work for non-random graphs such as Watts-strogatz/Barabasi-albert graphs that have a hub structure? Or does it implicitly assume an ‘expander’ like nature of the graph?
}\vspace{\comafter}

\noindent\textbf{Detailed Response 21:}
Our \textit{graph embedding} algorithm in Section VI computes latent coordinates for manifold graphs---graphs that can be reasonably assumed to be uniform discrete samples of a low-dimensional continuous manifold. 
We have added a detailed introduction of manifold graphs in Section III-A-1 of the revised manuscript.
Graphs with nodes of large differences in degrees do not fit our assumption of manifold graphs. 
With due respect to the reviewer, Watts-Strogatz graphs\footnote{https://en.wikipedia.org/wiki/Watts\%E2\%80\%93Strogatz\_model} and Barabasi-Albert graphs\footnote{https://en.wikipedia.org/wiki/Barab\%C3\%A1si\%E2\%80\%93Albert\_model} are not non-random graphs but random graphs, but with different probability distributions. 
We do not understand what the reviewer meant by ``an  `expander' like nature of the graph". 
\vspace{\resafter}




{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 22:}
The authors talk of ‘uniqueness’ in defining the objective in equation (31): is uniqueness more of importance that signal fidelity in practice — alternatively, can we have the same performance in recovery from both the graph structure types in Fig 6?
}\vspace{\comafter}

\noindent\textbf{Detailed Response 22:}
%There is actually no mention of ``uniqueness" in the paper in defining the objective in equation (38) of the revised manuscript (equation (31) of the original manuscript), so as authors we are confused what the reviewer is referring to.
We assume that by `uniqueness', the reviewer is referring the objective in equation (38) of the revised manuscript (equation (31) of the original manuscript) to compute latent coordinates  that includes the ``regularization" term $-\gamma \text{tr}(\P^\top \Q \P)$.
The problem is not about uniqueness, but computing a graph embedding consistent with the input graph structure in a latent space that is as low dimension as possible, which fits our basic assumption of a low-dimensional manifold.
By maximizing two-hop neighbor distances in addition to minimizing one-hop neighbor distances, we can better achieve that objective.

\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 23:}
On page 9. Sec-D: ‘Instead of orthogonality condition
…’ why is this proxy considered was not clear.
}\vspace{\comafter}

\noindent\textbf{Detailed Response 23:}
To simplify the overall technical presentation in the paper, in the revised manuscript we have removed the discussion on computing generalized eigenvectors to obtain latent coordinates for a manifold graph in favor of the simpler eigenvectors. 


\vspace{\resafter}



{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 24:}
In Experiments, Section A. Please explain clearly what graph is used, what is a node of the graph: is it a column of the image or the pixel?
}\vspace{\comafter}

\noindent\textbf{Detailed Response 24:}
We have provided a clearer explanation of the graph construction procedure in the revised manuscript. 
Specifically, we constructed a 4-connected 2D grid graph for an image, where each pixel is a graph node, and the collection of greyscale pixel values is the graph signal. 
\vspace{\resafter}



{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 25:}
I find it a bit strange to believe that the reconstructed images from the corrupted images in Figures 7(g) and Fig 8(a) can be so good, for any of the approaches used. Is the true signal information of the missing pixels used indirectly, perhaps through the weighted graph constructed by equation (4) and (5)? Please clarify.
}\vspace{\comafter}

\noindent\textbf{Detailed Response 25:}
We have released our MATLAB implementation of our image interpolation algorithm\footnote{https://www.eecs.yorku.ca/\~genec/software.html} so the reviewer can verify the shown performance in Fig.\;10 of the revised manuscript (Fig.\;7 in the original manuscript). 
We have provided a clearer explanation of the graph construction procedure for the image interpolation experiment in the revised manuscript. 
\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 26:}
I would also like to see the reconstruction performance of the missing patch on the Fig 7(a).
}\vspace{\comafter}

\noindent\textbf{Detailed Response 26:}
Fig.\;7 in the original manuscript has been replaced by Fig.\;10 in the revised manuscript, which better illustrates the performance of our proposed GGLR in image denoising and interpolation. 
Note that \textit{image inpainting} (where a large missing pixel patch is hallucinated) is not one of our current target applications and is thus out of scope.
\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 27:}
What is SSIM is not defined.
}\vspace{\comafter}

\noindent\textbf{Detailed Response 27:}
Structural similarity index measure (SSIM) \cite{wang2004image} is an exceedingly common objective image quality assessment metric in the image processing literature. 
Besides Peak Signal-to-Noise Ratio (PSNR), SSIM is by far the most prevalent image quality measure that is used in the imaging community today. 
We have provided appropriate reference in the revised manuscript. 
\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 28:}
From Table III, we notice that the performance gain on average does not noticeably exceed that of state of the art, in particular the SDGLR— which suggests that the gradient graph (central to the work) is not very useful. The authors should try to find settings where the SDGGLR is clearly advantageous over SDGLR. I believe the current examples do not show us the merit clearly.
}\vspace{\comafter}

\noindent\textbf{Detailed Response 28:}
With due respect to the reviewer, we do not believe this comment is evidence-based.
We observe from the revised Table III that (i) SDGGLR is always better than SDGLR for \textit{all} images and \textit{all} missing pixel percentages in PSNR, by up to 2.45dB in one case; (ii) SDGGLR is better than the computation-heavy model-based TGV by up to 1.88dB; and (iii) SDGGLR is significantly better deep-learning-based IRCNN when the number of missing pixels is large, \eg, by up to 16.93dB when 99\% of the pixels are missing. 
Further, the visual differences between SDGGLR and SDGLR in Fig.\;10 are stunningly obvious.
Thus, in our humble opinion, a fair-minded reader would indeed conclude that SDGGLR is useful compared to state-of-the-art methods in image restoration. 

\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 29:}
What is the average runtime for SDGLR in TABLE IV? Please include.
}\vspace{\comafter}

\noindent\textbf{Detailed Response 29:}
In the revised manuscript, we have addded the runtime for SDGLR in Table IV, which was slightly smaller than SDGGLR.

\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 30:}
It was also not clear to me why the title has Manifold in it, when clearly the entire work hinges on a graph, with given edges and adjacency — seems a bit misleading.
}\vspace{\comafter}

\noindent\textbf{Detailed Response 30:}
With due respect to the reviewer, this comment shows that the reviewer actually does not understand the central thesis of the paper: latent coordinates are crucial in computing manifold gradients to properly define GGLR and promote PWP signal reconstruction.
Without such node coordinates that are interpreted as discrete point coordinates of a low-dimensional continuous manifold in a latent space, planar / PWP signals cannot even be defined.
We apologize again for the unclear presentation in the original manuscript.
In the revised manuscript, we have rewritten the Introduction to emphasize the importance of latent coordinates in defining PWP signals, and added Section VI-A containing an explanation of why graph Laplacian alone cannot promote any notion of planar signals.
For graphs with latent coordinates (e.g., 2D images and 3D point clouds), manifold gradients can be readily computed to define GGLR following the development in Section\;IV. 
For graphs without latent coordinates, we propose a \textit{graph embedding} method to first compute these coordinates for manifold graphs in Section\;VI.
Thus, we believe the term ``manifold" is central to the paper's thesis and should be included in the paper title.

\vspace{\resafter}



{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 31:}
Some of the relevant works that use smoothness graph constraint are missing:

Xiaoyu Miao, Aimin Jiang, Tao Liu, Yanping Zhu, Hon Keung Kwan, ``Kernel Regression for Matrix-Variate Gaussian Distributed Signals Over Sample Graphs'', IEEE Transactions on Signal and Information Processing over Networks, vol.8, pp.726-738, 2022.

Hoi-To Wai, Yonina C. Eldar, Asuman E. Ozdaglar, Anna Scaglione, ``Community Inference From Partially Observed Graph Signals: Algorithms and Analysis'', IEEE Transactions on Signal Processing, vol.70, pp.2136-2151, 2022.

V. Borovitskiy, I, Azangulov, A. Terenin, et al. ``Matérn Gaussian processes on graphs,'' Proc. of Int. Conf. on Artificial Intelligence and Statistics (AISTATS), PMLR, pp. 2593-2601, 2021.

Arun Venkitaraman, Saikat Chatterjee, Peter Handel, ``Gaussian Processes Over Graphs'', ICASSP 2020 - 2020 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP), pp.5640-5644, 2020.

}\vspace{\comafter}

\noindent\textbf{Detailed Response 31:}
While we are thankful for the reviewer in providing a list of recent references, we find it hard to understand how they are directly related to our newly proposed prior GGLR in promoting PWP signal reconstruction.
In particular, the three papers titled ``Kernel Regression for Matrix-Variate Gaussian Distributed Signals over Sample Graphs", ``Mat\'{e}rn Gaussian Processes on Graphs", and ``Gaussian Processes over Graphs" are about building statistical / stochastic models (specifically, variants of Gaussian process) over graphs for prediction.
In contrast, our assumption of planar / PWP model is inherent \textit{deterministic} in nature, along the line of previous regularization approaches such as total variation (TV) \cite{chambolle1997image}, total generalized variation (TGV) \cite{bredies2010total, bredies2015tgv}, graph Laplacian regularizer (GLR) \cite{pang17} and graph total variation (GTV) \cite{elmoataz08,couprie13}, that are widely used in image restoration applications like 2D image denoising \cite{pang17}, JPEG dequantization \cite{liu17}, 3D point cloud denoising \cite{dinesh20}, etc. 
We do not find the paper titled ``Community Inference From Partially Observed Graph Signals: Algorithms and Analysis" relevant to our problem at all; the paper investigates the problem of identifying communities hidden in graph-structured data assumed to be low-pass filtered graph signals. 

For the sake of completeness, we have included two of three papers on Gaussian process in the discussion of related works.

\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Detailed Comment 32:}
I also feel that this work is more suited to IEEE TSIPN.
}\vspace{\comafter}


\noindent\textbf{Detailed Response 32:}
With due respect to the reviewer, the reviewer did not provide concrete evidence to support this opinion. 
The topic of our paper is clearly within the scope of TSP (there is an entire EDICS category named ``SIGNAL AND INFORMATION PROCESSING OVER GRAPHS" (SIPG)).
If the paper is of sufficient technical quality and within scope of TSP, how does one then determine the paper to be \textit{more} suitable for a different journal? 
Is it not the authors' decision to determine where to submit a manuscript for publication?
\vspace{\resafter}

==> response2reviewers_tsp/reviewer_AE.tex <==
{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 1:}
Please make sure that the comments from the three reviewers are comprehensively addressed in the revision if you wish to resubmit.

I concur with most of the reviewer's comments, particularly the technical ones. 
}\vspace{\comafter}

\noindent\textbf{Response 1:}
We thank the AE for a timely round of paper review.
We note that though many comments were provided (of which we are grateful), most were about textual clarifications with very few technical ones.

\vspace{\resafter}


{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 2:}
Statements such as ``provably promotes piecewise planar...'' do not make sense unless terms such as ``promotes'' and ``piecewise planar'' are properly defined in the first place. Indeed, one can only "prove" things about objects that have a concrete meaning; loose statements/insights cannot qualify for a mathematical proof. This happens in quite a few places where the authors have made statements without backing them with a proper justification.
}\vspace{\comafter}

\noindent\textbf{Response 2:}
First, with due respect to the AE, we do not state anywhere in the paper that GGLR ``provably promotes piecewise planar ...". 
We do state in the paper that GGLR ``\textit{provably} promotes planar signal reconstruction", which we indeed prove mathematically in Theorem 1 (Section IV-D of the revised manuscript). 
This is different from the statement ``we \textit{show / demonstrate} GGLR promotes PWP signal reconstruction".
For completeness, the definitions of planar and piecewise planar signals have been added in Section III-B of the revised manuscript. 

We have also added an explanation of the term ``promote" as a footnote in the Introduction: 

\vspace{0.1in}
\begin{quote}
By ``promote” we mean adding a non-negative signal prior $\text{Pr}(\x)$ to a minimization objective $f(\x)$ to bias the solution $\x$ towards small $\text{Pr}(\x)$.    
\end{quote}
See also our response to detailed comment 11 of reviewer 3 for a fuller explanation. 
Note that the terminology ``promote" is consistent with the GSP literature when discussing regularizers, for example, \cite{yankelevsky16}, \cite{mahmood18}, \cite{liu19depth}, Pg.41, Pg.50, Pg.146, Pg.147, Pg.148, Pg.149, Pg.150, Pg.152, Pg.204 in \cite{cheung21}.
Thus, we believe that our usage of the term ``promote" is well justified and consistent with the existing literature.

%In practice, one would introduce such regularization term if there is \textit{a priori} knowledge that the solution $\x$ is likely to have small $g(\x)$, e.g., $\text{Pr}(\x) \propto \exp(- g(\x))$. For imaging applications like 2D images and 3D point clouds, PWP is a common assumption as a signal prior \red{add refs}. For example, consider an image patch of a monotone background wall that is getting darker as the exposure to ambient light decreases \red{add image example}. Our proposal of GGLR is suitable for scenarios with prior signal knowledge that the sought signal is likely to be PWP.

Further, we believe that our three lemmas and four theorems in the revised paper are mathematically rigorous. 
If the AE believes these proofs are ``loose statements/insights" that ``cannot qualify for a mathematical proof", we humbly ask the AE to provide specific technical criticisms, and we will be happy to address them.
\vspace{\resafter}




{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 3:}
I think that the technical novelty is somewhat limited for TSP paper. As one of the reviewers pointed out, some of the theorems/lemmas are either straightforward or well-known.
}\vspace{\comafter}

\noindent\textbf{Response 3:}
With due respect to reviewer 2, we believe that reviewer 2's comment on novelty is an unjustified and gross over-simplification of our contributions in the paper with scant evidence provided, while overlooking a large fraction of the manuscript that was never mentioned. 
We note also that reviewer 2's criticism of our Theorem 3 in the revised manuscript (Lemma 2 in the original paper) as a known ordinary least square with ridge regularization is technically incorrect.
Please kindly see our response 2 and 3 to reviewer 2.
\vspace{\resafter}




{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 4:}
What I find particularly lacking is a solid understanding of how the proposed regularizer works and why it is able to outperform related graph regularizers. What would the analog of the regularizer for an analog signal f(x)? What does it measure? Since the Laplacian is already a second-order operator, the Laplacian of the gradient could be some form of third-order regularization. How does this relate to existing higher-order regularization schemes?
}\vspace{\comafter}


\noindent\textbf{Response 4:}
We have added a new Section IV-A titled ``Why Graph Laplacian cannot promote Planar Signals" in the revised manuscript, detailing why using the graph Laplacian to compute ``graph gradient" is inadequate to promote any notion of planar signals. 
The AE's statement ``since the Laplacian is already a second-order operator..." is actually an unfortunate but common misunderstanding of the graph Laplacian operator itself.
Further, we also explain the fallacy of reviewer 3's proposed regularizer $(\x-\A\x)^\top \L (\x-\A\x)$ as an alternative to promote smooth graph gradients.
Please kindly see our response 3 to reviewer 3 for details. 

As explained in the revised Introduction, \textit{to our knowledge there does not exist higher-order regularization for graph signals in the literature. 
In fact, we are the first in the GSP literature to propose one.}

\vspace{\resafter}




{\noindent\color{comment}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Comment 5:}
For the results on image interpolation and point cloud denoising, the authors should compare with state-of-the-art methods and not just related graph-based methods. After all, the practitioner would not so much care about how the method works but just the end result.
}\vspace{\comafter}


\noindent\textbf{Response 5:}
With due respect to the AE, \textit{we have already included non-graph based comparison methods for image interpolation}, including EPLL\cite{EPLLZoran2011}, IDBP\cite{tirer19}, GSC\cite{Zha2020}, IRCNN \cite{Zhang2017}.
See methods EPLL, IDBP, TGV, GSC, and IRCNN in Table III of the experimental Section VII.
For \textit{point cloud color denoising} (which is different from \textit{point cloud denoising} that focuses on denoising of point cloud coordinates), to our knowledge only graph-based methods exist in the literature to exploit available irregular 3D point geometry for denoising. 
If the AE is aware of non-graph-based point cloud color denoising methods, please kindly point them out and we will happy to conduct comparative experiments.

\vspace{\resafter}



==> spectrum.tex <==





\subsection{Eigen-pairs of $\cL^h$}

 


\subsubsection{First Eigen-pair for $\cL^h$}
\label{subsec:firstEigen}

Given $\L$ is PSD, we know $\cL = \F^{\top} \L \F$ is also PSD, and thus eigenvalues of $\cL$ are non-negative, \ie, $\lambda_i \geq 0$.
Given \eqref{eq:grad1}, one eigenvector $\v_1$ corresponding $\lambda_1 = 0$ for $\cL$ is constant vector $\1/\sqrt{K}$, since $\cL \1/\sqrt{K} = \L \F \1/\sqrt{K} = \0$. 

%\vspace{0.3in}

We examine the eigen-pairs of $\cL^h = \F^{\top} \L^h \F$. 
Denote by $\{(\theta_i,\u_i)\}$ the set of eigen-pairs for PSD symmetric $\L^h$.
Using the definition of Rayleigh quotient, we can write
\begin{align}
\u_i = \arg \min_{\x} \x^{\top} \L^h \x, 
~~~~~~\mbox{s.t.}~~
\x \perp \{\u_{k}\}_1^{i-1}
\end{align}
and $\theta_i = \u_i^{\top} \L^h \u_i$.
In particular, the first eigen-pair $(\theta_1,\u_1)$ for combinatorial graph Laplacian $\L^h$ is $(0, \1/\sqrt{K})$. 
Correspondingly, we can construct the first eigenvectors $\v_1$ and $\v_2$  corresponding to eigenvalue $0$ (of multiplicity 2) for $\cL^h$ as follows.
We first compute a vector $\r$ satisfying
\begin{align}
\1 = \F \, \r.
\label{eq:ev1}
\end{align}
(We defer the unit norm normalization of eigenvectors till later.)
\eqref{eq:ev1} is an under-determined linear system. 
We thus compute $\r = \F^+ \1$, where
$\F^+ = \F^{\top} (\F \F^{\top})^{-1}$ is the Moore-Penrose pseudo-inverse \red{add ref}.
Note the $\F^+$ is well defined, since $\F \F^{\top}$ is full rank by \eqref{eq:grad2} and thus invertible.
One can verify $\r$ satisfies \eqref{eq:ev1}: 
\begin{align}
\F \, \r = \F \F^+ \1 = 
\F \F^{\top} (\F \F^{\top} )^{-1} \1 
= \1.
\nonumber 
\end{align}

\begin{figure}[t]
\begin{center}
   \includegraphics[width=0.7\linewidth]{long version/firstEigen.png}
\end{center}
\vspace{-0.2in}
\caption{Illustration of constructing first eigenvectors $\v_1$ and $\v_2$ (blue arrows) from $\r$ (red arrow) in 2D space. Both $\v_1$ and $\v_2$ are on the line $c \r + d \1$, for $d \in \mathbb{R}$, where $c\r$ is inside the unit circle.} 
\label{fig:firstEigen}
\end{figure}

We next compute eigenvectors $\v_1$ and $\v_2$ of $\cL^h$ from $\r$. 
From \eqref{eq:grad1}, we see that $\v_i = c \r + d_i \1$ would ensure that $\F \v_i = \F c\r = c\1$.
However, $\v_1$ and $\v_2$ must in addition satisfy two constraints:
i) $\v_1$ and $\v_2$ must be unit norm, and ii) $\v_1$ and $\v_2$ must be mutually orthogonal.
We can now write the constraints mathematically as
\begin{align}
(c \r + d_1 \1)^{\top} (c \r + d_2 \1) &= 0 
\nonumber \\
\| c \r + d_1 \1 \|^2_2 = \| c \r + d_2 \1 \|^2_2 &= 1
\end{align}
We rewrite these constraints into
\begin{align}
c^2 \| \r\|^2_2 + c (d_1 + d_2) \sum_i r_i + d_1 d_2 K &= 0 
\nonumber \\
c^2 \| \r \|^2_2 + 2 c d_1 \sum_i r_i + d_1^2 K &= 1
\nonumber \\
c^2 \| \r \|^2_2 + 2 c d_2 \sum_i r_i + d_2^2 K &= 1
\label{eq:firstEigen}
\end{align}
See Fig.\;\ref{fig:firstEigen} for a 2D illustration of computed $\r$, scaled $c \r$, and eigenvectors $\v_1 = c\r + d_1 \1$ and $\v_2 = c\r + d_2 \1$ so that $\v_1^{\top} \perp \v_2$.
To solve for $c$, $d_1$ and $d_2$, we see that the corresponding equations for the three variables in \eqref{eq:firstEigen} are quadratic if the other variables are fixed.
(Second and third equations are the same, thus $d_1$ and $d_2$ are the two roots of the same quadratic equation.)
Thus, we first initialize $c$ so that
\begin{align}
\frac{K}{K \|r\|^2_2 - (\sum_i r_i)^2} \geq c^2
\end{align}
This ensures the computed $d_1$ and $d_2$ using \eqref{eq:firstEigen} are real numbers.
We then solve for $d_1$ and $d_2$ in order, and solve for $c$ while fixing $d_1$ and $d_2$.
We repeat the above procedure until convergence.

\begin{figure}[t]
\begin{center}
   \includegraphics[width=0.49\linewidth]{long version/4nodeDerivedEigen.png}
   %\hspace{0.05in}
   \includegraphics[width=0.49\linewidth]{long version/4nodeEigen.png}
\end{center}
\vspace{-0.2in}
\caption{Examples of derived first eigenvectors (left) and computed eigenvectors (right) for a 4-node graph.} 
\label{fig:eigenEx}
\end{figure}

\begin{figure}[t]
\begin{center}
   \includegraphics[width=0.49\linewidth]{long version/5nodeEigenU.png}
   %\hspace{0.05in}
   \includegraphics[width=0.49\linewidth]{long version/5nodeEigen.png}
\end{center}
\vspace{-0.2in}
\caption{Examples of computed eigenvectors of $\L^h$ (left) and $\cL^h$ (right) for a 5-node graph.} 
\label{fig:eigenEx2}
\end{figure}

See Fig.\;\ref{fig:eigenEx}(left) for an example of derived first eigenvectors for a 4-node graph using our proposed procedure, and Fig.\;\ref{fig:eigenEx}(right) for eigenvectors of the same Laplacian $\cL^h$ via eigen-dcomposition.
We observe that in both cases, the first eigenvectors $\v_1$ and $\v_2$ are linear.
In the first case, $\v_2$ is a DC shift $d\1$ of $\v_1$. 


\subsubsection{Subsequent Eigen-pairs for $\cL^h$}

We next examine eigen-pairs for $\cL^h$ corresponding to $(\theta_i,\u_i)$ for $i \geq 2$. 
Corresponding to each $\u_i$, we construct an eigen-vector $\v_{i+1}$ as follows. 
We first compute $\r = \F^{+} \u_i$. We then select $\v_{i+1} = c_i \r$, so that $\| \v_{i+1} \|^2_2 = 1$; 
\ie, 
\begin{align}
\|c_i \F^+ \u_i \|^2_2 &= 
c_i^2 \u_i^{\top} (\F^+)^{\top} \F^+ \u_i 
= 1 
\nonumber \\
c_i &= \frac{1}{(\u_i^{\top} (\F^+)^{\top} \F^+ \u_i)^{1/2}}
\end{align}
We first prove that $\v_{i+1} \perp \{\v_k\}_{k=1}^{i}$.
We prove this in two separate cases. 
For $3 \leq k \leq i$,
\begin{align}
\v_{i+1}^{\top} \v_k &= c_i c_{k-1}
\u_i^{\top} (\F^{+})^{\top} \F^+ \u_{k-1} 
\nonumber \\
&= c_i c_{k-1} \u_i^{\top} 
(\F \F^{\top})^{-1}
\F
\F^{\top} (\F \F^{\top})^{-1} \u_{k-1} 
\nonumber \\
&= c_i c_{k-1} \text{tr}( (\F \F^{\top})^{-1} \u_{k-1} \u_i^{\top} )
\stackrel{(a)}{\leq} c_i c_{k-1} \sum_j \alpha_j \beta_j
\nonumber 
\end{align}
where $\alpha_j$'s and $\beta_j$'s are the eigenvalues of $(\F \F^{\top})^{-1}$ and $\u_{k-1} \u_i^{\top}$, respectively, and $(a)$ is due to Von Neumann's trace inequality \red{add ref}.  
The outer-product matrix $\u_{k-1} \u_i^{\top}$ has rank no larger than $1$, thus $\beta_j = 0$, for $1 \leq k \leq K-1$. 
We know also that $\text{tr}(\u_{k-1} \u_i^{\top}) = \u_i^{\top} \u_{k-1} = 0 = \sum_j \beta_j$. 
Thus, we conclude that $\beta_j = 0, \forall j$, and therefore $\v_{i+1}^{\top} \v_k = 0$ for $3 \leq k \leq i$. 

Consider next the case when $1 \leq k \leq 2$. 
We know eigenvectors computed in Section\;\ref{subsec:firstEigen} are of the form $\v_k = c \r + d \1$. 
Thus
\begin{align}
\v_{i+1}^{\top} \v_k &= c_i \u_i^{\top} (\F^{+})^{\top} (c (\F^+ \1) + d \1) 
\nonumber \\
&= c_i c\, \u_i^{\top} (\F \F^{\top} )^{-1} \F \F^{\top} (\F \F^{\top} )^{-1} \1 +
c_i d\, \u_i^{\top} (\F^+)^{\top} \1
\nonumber \\
&= c_i c\,\text{tr}((\F \F^{\top})^{-1} \1 \u_i^{\top}) + c_i d\, \text{tr}((\F^+)^{\top} \1 \u_i^{\top}) \stackrel{(a)}{=} 0.
\nonumber 
\end{align}
where $(a)$  is true due again to Von Neumann's trace inequality and that $\u_i \perp \1$. 
Therefore, we can conclude that $\v_{i+1} \perp \{\v_k\}^i_{k=1}$. 



